Private Function Computation for Noncolluding Coded Databases

Private computation in a distributed storage system (DSS) is a generalization of the private information retrieval (PIR) problem. In such setting a user wishes to compute a function of $f$ messages stored in $n$ noncolluding coded databases, i.e., databases storing data encoded with an $[n,k]$ linear storage code, while revealing no information about the desired function to the databases. We consider the problem of private polynomial computation (PPC). In PPC, a user wishes to compute a multivariate polynomial of degree at most $g$ over $f$ variables (or messages) stored in multiple databases. First, we consider the private computation of polynomials of degree $g=1$, i.e., private linear computation (PLC) for coded databases. In PLC, a user wishes to compute a linear combination over the $f$ messages while keeping the coefficients of the desired linear combination hidden from the database. For a linearly encoded DSS, we present a capacity-achieving PLC scheme and show that the PLC capacity, which is the ratio of the desired amount of information and the total amount of downloaded information, matches the maximum distance separable coded capacity of PIR for a large class of linear storage codes. Then, we consider private computation of higher degree polynomials, i.e., $g>1$. For this setup, we construct two novel PPC schemes. In the first scheme, we consider Reed-Solomon coded databases with Lagrange encoding, which leverages ideas from recently proposed star-product PIR and Lagrange coded computation. The second scheme considers the special case of coded databases with systematic Lagrange encoding. Both schemes yield improved rates, while asymptotically, as $f\rightarrow \infty$, the systematic scheme gives a significantly better computation retrieval rate compared to all known schemes up to some storage code rate that depends on the maximum degree of the candidate polynomials.

==> Revision 1/Algorithm_1.tex <==

\renewcommand{\baselinestretch}{0.95}
\begin{algorithm}[htbp]
  \caption{\texttt{Q-Gen}}
  \label{alg:generation_QuerySet}
  \SetInd{0.35em}{0.35em}
  \small
  \SetKwFunction{InitialRound}{Initial-Round}
  \SetKwFunction{Partition}{Partition}
  \SetKwFunction{DesiredQ}{Desired-Q}
  \SetKwFunction{ExploitSI}{Exploit-SI}
  \SetKwFunction{SetAddition}{SetAddition}
  \SetKwFunction{MSym}{M-Sym}  
  \SetKwInOut{Input}{Input}
  \SetKwInOut{Output}{Output}
  \SetKwComment{Comment}{$\triangleright$\ }{}{}
  \DontPrintSemicolon
  
  \Input{$v$, $\mu$, $\kappa$, $\nu$, $n$, $\mat{A}_{\kappa\times n}$, and $\mat{B}_{(\nu-\kappa)\times n}$}
  \Output{${Q}^{(v)}_1,\ldots,{Q}^{(v)}_n$}
  %$Q^{(v)}_j\leftarrow\emptyset$, $j\in[1:n]$\;
  \For{$\tau\in [\mu]$}{    
  $Q^{(v)}_j(\mathcal{D};\tau) \leftarrow\emptyset$, $Q^{(v)}_j(\mathcal{U};\tau) \leftarrow\emptyset$,  $j\in [n]$\;
    $\alpha_{\tau}\leftarrow\kappa^{\mu-1}+\sum_{h=1}^{\tau-1}\binom{\mu-1}{h}\kappa^{\mu-(h+1)}(\nu-\kappa)^{h}$\;
    \Comment{\b Generate query sets for the initial round}
    \If{$\tau=1$}{
      \For{$u\in [\nu]$}{
        \For{$j\in \set{S}(u|\mat{A}_{\kappa\times n})$}{
          $Q^{(v)}_j(u,\set{D};\tau),Q^{(v)}_j(u,\set{U};\tau)\leftarrow\InitialRound(u,\alpha_\tau,j,v,\tau)$\;     
        }      
      }
    }
    \Comment{\b Generate query sets for the following rounds $\tau>1$}
    \Else{
      \For{$u\in [\nu]$}{
        \Comment{\b Generate desired symbols for the following rounds $\tau>1$}
        \For{$j\in \set{S}(u|\mat{A}_{\kappa\times n})$}{
          $Q^{(v)}_j(u,\set{D};\tau)\leftarrow\DesiredQ(u,\alpha_\tau,j,v,\tau)$\;}
        \Comment{\b Generate side information for the following rounds $\tau>1$}
        \For{$j\in\set{S}(u|\mat{B}_{(\nu-\kappa)\times n})$}{
          $Q^{(v)}_j(u,\set{U};\tau-1)\leftarrow
          \ExploitSI(u,Q^{(v)}_1(u,\mathcal{U},\tau-1),\ldots,Q^{(v)}_n(u,\mathcal{U},\tau-1),j,v,\tau)$\;}
      }
      \Comment{\b Generate the final desired query sets for the following rounds $\tau>1$}
        \For{$j\in [n]$}{
          $\tilde{Q}^{(v)}_j(\set{U};\tau-1)\leftarrow\bigcup\limits_{i\in [\nu-\kappa] }Q^{(v)}_j(b_{i,j},\set{U};\tau-1)$\;
          $\tilde{Q}^{(v)}_j(1,\set{U};\tau-1),\ldots, \tilde{Q}^{(v)}_j(\kappa,\set{U};\tau-1) \leftarrow
          \Partition\bigl(\tilde{Q}^{(v)}_j(\set{U};\tau-1)\bigr)$\;
          \For{$i\in [\kappa]$}{
            $Q^{(v)}_j(a_{i,j},\set{D};\tau)\leftarrow
            \SetAddition\bigl(Q_j^{(v)}(a_{i,j},\set{D};\tau),\tilde{Q}^{(v)}_j(i,\set{U};\tau-1)\bigr)$\;          
          }      
        }
      \Comment{\b Generate the query sets of undesired symbols by forcing message symmetry for the following rounds $\tau>1$}  
      \For{$u\in [\nu] $}{
        \For{$j\in\set{S}(u|\mat{A}_{\kappa\times n})$}{
          $Q^{(v)}_j(u,\set{U};\tau)\leftarrow\MSym\bigl(Q_j^{(v)}(u,\set{D};\tau),j,v,\tau\bigr)$\;}
      }
    }
      \For{$u\in [\nu]$}{
        \For{$j\in \set{S}(u|\mat{A}_{\kappa\times n})$}{
          $Q^{(v)}_j(\set{D};\tau)\leftarrow Q^{(v)}_j(\set{D};\tau) \cup Q^{(v)}_j(u,\set{D};\tau)$\;
          $Q^{(v)}_j(\set{U};\tau)\leftarrow Q^{(v)}_j(\set{U};\tau) \cup Q^{(v)}_j(u,\set{U};\tau)$\;
        }
      }
  }  
  \For{$j\in [n]$}{
    $Q^{(v)}_j\leftarrow\bigcup\limits_{\tau\in [\mu]}\Bigl(Q^{(v)}_j(\set{D};\tau)\cup 
    Q^{(v)}_j(\set{U};\tau)\Bigr)$\;
  }
\end{algorithm}
\renewcommand{\baselinestretch}{1}


==> Revision 1/Algorithm_2.tex <==
\begin{algorithm}[htbp]
  \caption{\texttt{Initial-Round}}
  \label{alg:initial-round}
  \SetInd{0.35em}{0.35em}
  \small
  \SetKwFunction{new}{new}
  \SetKwInOut{Input}{Input}
  \SetKwInOut{Output}{Output}
  \SetKwComment{Comment}{$\triangleright$\ }{}
  \DontPrintSemicolon	 
  
  \Input{$u$, $\alpha_\tau$, $j$, $v$, and $\tau$}
  \Output{$\varphi^{(v)}(u,\set{D};\tau), \varphi^{(v)}(u,\set{U};\tau)$}
  
  $\varphi^{(v)}(u,\set{D};\tau)\leftarrow\emptyset$, $\varphi^{(v)}(u,\set{U};\tau)\leftarrow\emptyset$\;
  % \Comment{\textcolor{blue}{Generate query set for the initial round}}
  \For{$l\in [\alpha_{\tau}]$}{
    $\varphi^{(v)}(u,\set{D};\tau)\leftarrow\varphi^{(v)}(u,\set{D};\tau)\cup\bigl\{U^{(v)}_{({u}-1)
      \cdot\alpha_\tau+l,j}\bigr\}$\;
    $\varphi^{(v)}(u,\set{U};\tau)\leftarrow\varphi^{(v)}(u,\set{U};\tau)\ \cup$
    $%\phantom{abcdefghijklmn}
    \left(\bigcup\limits_{v'=1}^{\mu}\bigl\{U^{(v')}_{({u}-1)\cdot\alpha_\tau+l,j}\bigr\}
      \setminus\bigl\{U^{(v)}_{({u}-1)\cdot\alpha_\tau+l,j}\bigr\}\right)$\;
  }
\end{algorithm}



==> Revision 1/Algorithm_3.tex <==
\begin{algorithm}[htbp]
  \caption{\texttt{Desired-Q}}
  \label{alg:Desired-setQ_following-rounds}
  \SetInd{0.35em}{0.35em}
  \small
  \SetKwInOut{Input}{Input}
  \SetKwInOut{Output}{Output}
  \SetKwComment{Comment}{$\triangleright$\ }{}
  \DontPrintSemicolon	   
  \Input{$u$, $\alpha_\tau$, $j$, $v$, and $\tau$}
  \Output{$\varphi^{(v)}(u,\set{D};\tau)$}  
  $\varphi^{(v)}(u,\set{D};\tau)\leftarrow\emptyset$\;
  % \Comment{\b Generate the query set of desired symbols w.r.t.\ a particular $u$ for the following rounds $\tau>1$}
  \For{$l\in[\alpha_{\tau-1}:\alpha_\tau-1]$}{
    $\varphi^{(v)}(u,\set{D};\tau)\leftarrow\varphi^{(v)}(u,\set{D};\tau)
    \cup\bigl\{U^{(v)}_{l\cdot\nu+{u},j}\bigr\}$\;
  }
\end{algorithm}


==> Revision 1/Algorithm_4.tex <==
\begin{algorithm}[htbp!]
  \caption{\texttt{Exploit-SI}}
  \label{alg:Exploit-SI}
  \SetInd{0.35em}{0.35em}
  \small
  \SetKwFunction{Reproduce}{Reproduce}
  \SetKwInOut{Input}{Input}
  \SetKwInOut{Output}{Output}
  \SetKwComment{Comment}{$\triangleright$\ }{}
  \DontPrintSemicolon	 
  
  \Input{$u$, $Q^{(v)}_1(u,\set{U};\tau-1),\ldots,Q^{(v)}_n(u,\set{U};\tau-1)$, $j$, $v$, and $\tau$} %, %$j\in [1:n]\setminus\{j\}$}
  \Output{$\varphi^{(v)}(u,\set{U};\tau-1)$}
  
  $\varphi^{(v)}(u,\set{U};\tau-1)\leftarrow\emptyset$\;  
  \For{$i\in [\kappa]$}{
    \For{$j'\in [n]\setminus\{j\}$}{
      \If{$u=a_{i,j'}$}{
        $\varphi^{(v)}(u,\set{U};\tau-1)\leftarrow\Reproduce(j,Q^{(v)}_{j'}(u,\set{U};\tau-1))$\;
        break\;
      }
    }
  }
\end{algorithm}	






==> Revision 1/Algorithm_5.tex <==
\begin{algorithm}[htbp!]
  \caption{\texttt{M-Sym}}
  \label{alg:message-symmetry}
  \SetInd{0.35em}{0.35em}
  \small
  \SetKwFunction{Msym}{M-sym}
  \SetKwFunction{Lexico}{Lexico}
  \SetKwInOut{Input}{Input}
  \SetKwInOut{Output}{Output}
  \SetKwComment{Comment}{$\triangleright$\ }{}
  \DontPrintSemicolon	 
  
  \Input{$Q^{(v)}_j(u,\set{D};\tau)$, $j$, $v$, and $\tau$}
  \Output{$\varphi^{(v)}(u,\set{U};\tau)$}
  
  $\varphi^{(v)}(u,\set{U};\tau)\leftarrow\emptyset$\;
  \For{$(v_1,\ldots,v_\tau)\in\Lexico(\Pi_\tau)$, $v\notin \{v_1,\ldots,v_\tau \}$}{
    $\varphi^{(v)}(u,\set{U};\tau)\leftarrow\varphi^{(v)}(u,\set{U};\tau)\cup
    \bigl\{U^{(v_1)}_{i_1,j}+\ldots+U^{(v_\tau)}_{i_\tau,j}\bigr\}$ $\textnormal{ such that }
    \forall\,z\in [\tau] $, $\exists\,U^{(v)}_{i_z,j}+\sum\limits_{\substack{x\in [\tau]\\ x\neq z}}
    U^{(v_x)}_{\ast,j}\in Q^{(v)}_j(u,\set{D};\tau)$\;
  }
\end{algorithm}	




==> Revision 1/fig/CodedPMC_N7_K2_d2_trueAllsys.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{1.00000,0.00000,1.00000}%
%
\begin{tikzpicture}

\begin{axis}[%
width=4.967in, 
height=4.329in,
at={(1.95in,0.779in)},
scale only axis,
separate axis lines,
every outer x axis line/.append style={black},
every x tick label/.append style={font=\color{black}},
every x tick/.append style={black},
xmin=1,
xmax=8,
xtick={1, 2, 3, 4, 5, 6, 7, 8},
xlabel={Number of messages $f$},
every outer y axis line/.append style={black},
every y tick label/.append style={font=\color{black}},
every y tick/.append style={black},
ymin=0.1,
ymax=0.6,
ytick={0, 0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8},
ylabel={PMC rate $\const{R}$},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
grid style={gray,opacity=0.75,dotted},
grid style={gray,opacity=0.75,dotted},
legend style={legend cell align=left, align=left, draw=white!15!black, fill=white}
]

\addplot [color=mycolor1, line width=1.5pt, mark=square*, mark options={mycolor1,fill=white}]
table[row sep=crcr]{%
	1	0.579380164285695\\
	2	0.450629016666652\\
	3	0.423725791791031\\
	4	0.416619279559735\\
	5	0.414632421594621\\
	6	0.414068223886962\\
	7	0.41390730644965\\
	8	0.41386135300907\\
};
\addlegendentry{\small Converse bound (Thm.~\ref{thm:converse_bound})}


\addplot [color=red, mark=*,  line width=1.5pt,mark options={red,fill=white}]
  table[row sep=crcr]{%
1	0.38625344285713\\
2	0.237915473653148\\
3	0.22168944039731\\
4	0.220738565673707\\
5	0.220716455604713\\
6	0.220716253803995\\
7	0.220716253062335\\
8	0.220716253061218\\
};
\addlegendentry{\small RS-L (Thm.~\ref{thm:PMCrate_LagrangeCoded-DSS})} 

\addplot [color=black, line width=1.5pt, mark options={black,fill=white}]
  table[row sep=crcr]{%
1	0.220716253061217\\
2	0.220716253061217\\
3	0.220716253061217\\
4	0.220716253061217\\
5	0.220716253061217\\
6	0.220716253061217\\
7	0.220716253061217\\
8	0.220716253061217\\
};
\addlegendentry{\small PPC scheme \cite{RavivKarpuk19_2}}

\addplot [color=blue, line width=1.5pt, mark=diamond*, mark options={blue,fill=white}]
table[row sep=crcr]{%
	1	0.413842974489782\\
	2	0.26312498378038\\
	3	0.248958414239293\\
	4	0.248316449804179\\
	5	0.248305848852434\\
	6	0.248305784839244\\
	7	0.248305784693995\\
	8	0.248305784693869\\
};
\addlegendentry{\small Sys.~RS-L (Thm.~\ref{thm:RS_PPC_rate})} 

\addplot [color=green, line width=1.5pt, mark options={green,fill=white}]
table[row sep=crcr]{%
	1	0.165537189795913\\
	2	0.165537189795913\\
	3	0.165537189795913\\
	4	0.165537189795913\\
	5	0.165537189795913\\
	6	0.165537189795913\\
	7	0.165537189795913\\
	8	0.165537189795913\\
};
\addlegendentry{\small Sys.~PPC scheme \cite{Karpuk18_1}} 

\end{axis}
\end{tikzpicture}%

==> Revision 1/fig/CodedPMC_N7_K2_d2_trueUnparlsys.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{1.00000,0.00000,1.00000}%
%
\begin{tikzpicture}

\begin{axis}[%
width=4.967in, 
height=4.329in,
at={(1.95in,0.779in)},
scale only axis,
separate axis lines,
every outer x axis line/.append style={black},
every x tick label/.append style={font=\color{black}},
every x tick/.append style={black},
xmin=1,
xmax=8,
xtick={1, 2, 3, 4, 5, 6, 7},
xlabel={Number of messages $f$},
every outer y axis line/.append style={black},
every y tick label/.append style={font=\color{black}},
every y tick/.append style={black},
ymin=0.2,
ymax=1,
%ytick={0, 0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8},
ylabel={PMC rate $\const{R}$},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
grid style={gray,opacity=0.75,dotted},
legend style={legend cell align=left, align=left, draw=white!15!black, fill=white}
]
\addplot [color=mycolor1, line width=1.5pt, mark=square*, mark options={mycolor1,fill=white}]
table[row sep=crcr]{%
	1	1\\
	2	0.70444313178854\\
	3	0.662386825413105\\
	4	0.651277612408273\\
	5	0.64817166850409\\
	6	0.647289689791154\\
	7	0.647038136563762\\
	8	0.64696630012092\\
};
\addlegendentry{\small Converse bound (Thm.~\ref{thm:converse_bound})}

\addplot [color=red, mark=*,  line width=1.5pt,mark options={red,fill=white}]
table[row sep=crcr]{%
	1	0.666666666666666\\
	2	0.422665879073124\\
	3	0.356064971634178\\
	4	0.345683730333475\\
	5	0.345048318405106\\
	6	0.34503350636826\\
	7	0.345033371169571\\
	8	0.345033370672687\\
};
\addlegendentry{\small RS-L (Thm.~\ref{thm:PMCrate_LagrangeCoded-DSS})} 

\addplot [color=black, line width=1.5pt, mark options={black,fill=white}]
  table[row sep=crcr]{%
1	0.345033370671938\\
2	0.345033370671938\\
3	0.345033370671938\\
4	0.345033370671938\\
5	0.345033370671938\\
6	0.345033370671938\\
7	0.345033370671938\\
8	0.345033370671938\\
};
\addlegendentry{\small PPC scheme \cite{RavivKarpuk19_2}}

\addplot [color=blue, line width=1.5pt, mark=diamond*, mark options={blue,fill=white}]
table[row sep=crcr]{%
	1	0.714285714\\
	2	0.462098264292774\\
	3	0.39710860465152\\
	4	0.388569987168796\\
	5	0.388169210702191\\
	6	0.388162582124122\\
	7	0.388162542096833\\
	8	0.388162542006009\\
};
\addlegendentry{\small Sys.~RS-L (Thm.~\ref{thm:RS_PPC_rate})} 

\addplot [color=green, line width=1.5pt, mark options={green,fill=white}]
table[row sep=crcr]{%
	1	0.258775028003953\\
	2	0.258775028003953\\
	3	0.258775028003953\\
	4	0.258775028003953\\
	5	0.258775028003953\\
	6	0.258775028003953\\
	7	0.258775028003953\\
	8	0.258775028003953\\
};
\addlegendentry{\small Sys.~PPC scheme \cite{Karpuk18_1}}


\end{axis}
\end{tikzpicture}%

==> Revision 1/fig/CodedPMC_k20_g2_f10_compare.tex <==

\definecolor{mycolor1}{rgb}{0.00000,1.00000,1.00000}%
\definecolor{mycolor2}{rgb}{0.60000,0.00000,0.60000}%
%


\begin{tikzpicture}
%\pgfplotsset{every tick label/.append style={font=\small}}
\begin{axis}[%
width=4.967in,
height=4.329in,
%width=12.5cm,
%height=10.0cm,
at={(1.95in,0.779in)},
%at={(1.387in,0.821in)},
xmin=0,
xmax=0.5, 
xlabel={Storage code rate $\alpha=k/n$},
xlabel style={
	yshift=0.5ex,
	name=label},
xmajorgrids,
xtick={0,0.05,0.1,0.15,0.2,0.25,0.3,0.35,0.4,0.45,0.5},
ymajorgrids,
ymin=0.0, %ymin=0.1,
max space between ticks=20pt,
ymax=0.5, %ymax=0.8,
ylabel={PMC rate $\const{R}$},
ylabel style={
	yshift=-1.0ex,
	name=label},
ytick={0,0.05,0.1,0.15,0.2,0.25,0.3,0.35,0.4,0.45,0.5},
grid style={gray,opacity=0.75,dotted},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
scale only axis,
every outer x axis line/.append style={black},
every x tick label/.append style={font=\color{black}},
every x tick/.append style={black},
every outer y axis line/.append style={black},
every y tick label/.append style={font=\color{black}},
every y tick/.append style={black},
legend style={legend cell align=left, align=left, draw=white!15!black, fill=white}
]

\addplot [color=mycolor2, dashed, line width=1.5pt, mark=diamond*, mark options={solid, mycolor2}]
table[row sep=crcr]{%
0.05	0.1\\
0.050125313283208	0.1\\
0.050251256281407	0.1\\
0.0503778337531486	0.1\\
0.0505050505050505	0.1\\
0.0506329113924051	0.1\\
0.050761421319797	0.1\\
0.0508905852417303	0.1\\
0.0510204081632653	0.1\\
0.051150895140665	0.1\\
0.0512820512820513	0.1\\
0.051413881748072	0.1\\
0.0515463917525773	0.1\\
0.0516795865633075	0.1\\
0.0518134715025907	0.1\\
0.051948051948052	0.1\\
0.0520833333333333	0.1\\
0.0522193211488251	0.1\\
0.0523560209424084	0.1\\
0.05249343832021	0.1\\
0.0526315789473684	0.1\\
0.0527704485488127	0.1\\
0.0529100529100529	0.1\\
0.0530503978779841	0.1\\
0.0531914893617021	0.1\\
0.0533333333333333	0.1\\
0.053475935828877	0.1\\
0.0536193029490617	0.1\\
0.0537634408602151	0.1\\
0.0539083557951483	0.1\\
0.0540540540540541	0.1\\
0.0542005420054201	0.1\\
0.0543478260869565	0.1\\
0.0544959128065395	0.1\\
0.0546448087431694	0.1\\
0.0547945205479452	0.1\\
0.0549450549450549	0.1\\
0.0550964187327824	0.1\\
0.0552486187845304	0.1\\
0.0554016620498615	0.1\\
0.0555555555555556	0.1\\
0.0557103064066852	0.1\\
0.0558659217877095	0.1\\
0.0560224089635854	0.1\\
0.0561797752808989	0.1\\
0.0563380281690141	0.1\\
0.0564971751412429	0.1\\
0.056657223796034	0.1\\
0.0568181818181818	0.1\\
0.056980056980057	0.1\\
0.0571428571428571	0.1\\
0.0573065902578797	0.1\\
0.0574712643678161	0.1\\
0.0576368876080692	0.1\\
0.0578034682080925	0.1\\
0.0579710144927536	0.1\\
0.0581395348837209	0.1\\
0.0583090379008746	0.1\\
0.0584795321637427	0.1\\
0.0586510263929619	0.1\\
0.0588235294117647	0.1\\
0.0589970501474926	0.1\\
0.0591715976331361	0.1\\
0.0593471810089021	0.1\\
0.0595238095238095	0.1\\
0.0597014925373134	0.1\\
0.0598802395209581	0.1\\
0.0600600600600601	0.1\\
0.0602409638554217	0.1\\
0.0604229607250755	0.1\\
0.0606060606060606	0.1\\
0.060790273556231	0.1\\
0.0609756097560976	0.1\\
0.0611620795107034	0.1\\
0.0613496932515337	0.1\\
0.0615384615384615	0.1\\
0.0617283950617284	0.1\\
0.0619195046439628	0.1\\
0.062111801242236	0.1\\
0.0623052959501558	0.1\\
0.0625	0.1\\
0.0626959247648903	0.1\\
0.0628930817610063	0.1\\
0.0630914826498423	0.1\\
0.0632911392405063	0.1\\
0.0634920634920635	0.1\\
0.0636942675159236	0.1\\
0.0638977635782748	0.1\\
0.0641025641025641	0.1\\
0.0643086816720257	0.1\\
0.0645161290322581	0.1\\
0.0647249190938511	0.1\\
0.0649350649350649	0.1\\
0.0651465798045603	0.1\\
0.065359477124183	0.1\\
0.0655737704918033	0.1\\
0.0657894736842105	0.1\\
0.066006600660066	0.1\\
0.0662251655629139	0.1\\
0.0664451827242525	0.1\\
0.0666666666666667	0.1\\
0.0668896321070234	0.1\\
0.0671140939597315	0.1\\
0.0673400673400673	0.1\\
0.0675675675675676	0.1\\
0.0677966101694915	0.1\\
0.0680272108843537	0.1\\
0.068259385665529	0.1\\
0.0684931506849315	0.1\\
0.0687285223367698	0.1\\
0.0689655172413793	0.1\\
0.069204152249135	0.1\\
0.0694444444444444	0.1\\
0.0696864111498258	0.1\\
0.0699300699300699	0.1\\
0.0701754385964912	0.1\\
0.0704225352112676	0.1\\
0.0706713780918728	0.1\\
0.0709219858156028	0.1\\
0.0711743772241993	0.1\\
0.0714285714285714	0.1\\
0.0716845878136201	0.1\\
0.0719424460431655	0.1\\
0.0722021660649819	0.1\\
0.072463768115942	0.1\\
0.0727272727272727	0.1\\
0.072992700729927	0.1\\
0.0732600732600733	0.1\\
0.0735294117647059	0.1\\
0.0738007380073801	0.1\\
0.0740740740740741	0.1\\
0.0743494423791822	0.1\\
0.0746268656716418	0.1\\
0.0749063670411985	0.1\\
0.075187969924812	0.1\\
0.0754716981132075	0.1\\
0.0757575757575758	0.1\\
0.0760456273764259	0.1\\
0.0763358778625954	0.1\\
0.0766283524904215	0.1\\
0.0769230769230769	0.1\\
0.0772200772200772	0.1\\
0.0775193798449612	0.1\\
0.0778210116731518	0.1\\
0.078125	0.1\\
0.0784313725490196	0.1\\
0.078740157480315	0.1\\
0.0790513833992095	0.1\\
0.0793650793650794	0.1\\
0.0796812749003984	0.1\\
0.08	0.1\\
0.0803212851405622	0.1\\
0.0806451612903226	0.1\\
0.0809716599190283	0.1\\
0.0813008130081301	0.1\\
0.0816326530612245	0.1\\
0.0819672131147541	0.1\\
0.0823045267489712	0.1\\
0.0826446280991736	0.1\\
0.0829875518672199	0.1\\
0.0833333333333333	0.1\\
0.0836820083682008	0.1\\
0.0840336134453782	0.1\\
0.0843881856540084	0.1\\
0.0847457627118644	0.1\\
0.0851063829787234	0.1\\
0.0854700854700855	0.1\\
0.0858369098712446	0.1\\
0.0862068965517241	0.1\\
0.0865800865800866	0.1\\
0.0869565217391304	0.1\\
0.0873362445414847	0.1\\
0.087719298245614	0.1\\
0.0881057268722467	0.1\\
0.0884955752212389	0.1\\
0.0888888888888889	0.1\\
0.0892857142857143	0.1\\
0.0896860986547085	0.1\\
0.0900900900900901	0.1\\
0.0904977375565611	0.1\\
0.0909090909090909	0.1\\
0.091324200913242	0.1\\
0.0917431192660551	0.1\\
0.0921658986175115	0.1\\
0.0925925925925926	0.1\\
0.0930232558139535	0.1\\
0.0934579439252336	0.1\\
0.0938967136150235	0.1\\
0.0943396226415094	0.1\\
0.0947867298578199	0.1\\
0.0952380952380952	0.1\\
0.0956937799043062	0.1\\
0.0961538461538462	0.1\\
0.0966183574879227	0.1\\
0.0970873786407767	0.1\\
0.0975609756097561	0.1\\
0.0980392156862745	0.1\\
0.0985221674876847	0.1\\
0.099009900990099	0.1\\
0.0995024875621891	0.1\\
0.1	0.1\\
0.100502512562814	0.1\\
0.101010101010101	0.1\\
0.101522842639594	0.1\\
0.102040816326531	0.1\\
0.102564102564103	0.1\\
0.103092783505155	0.1\\
0.103626943005181	0.1\\
0.104166666666667	0.1\\
0.104712041884817	0.1\\
0.105263157894737	0.1\\
0.105820105820106	0.1\\
0.106382978723404	0.1\\
0.106951871657754	0.1\\
0.10752688172043	0.1\\
0.108108108108108	0.1\\
0.108695652173913	0.1\\
0.109289617486339	0.1\\
0.10989010989011	0.1\\
0.110497237569061	0.1\\
0.111111111111111	0.1\\
0.111731843575419	0.1\\
0.112359550561798	0.1\\
0.112994350282486	0.1\\
0.113636363636364	0.1\\
0.114285714285714	0.1\\
0.114942528735632	0.1\\
0.115606936416185	0.1\\
0.116279069767442	0.1\\
0.116959064327485	0.1\\
0.117647058823529	0.1\\
0.118343195266272	0.1\\
0.119047619047619	0.1\\
0.119760479041916	0.1\\
0.120481927710843	0.1\\
0.121212121212121	0.1\\
0.121951219512195	0.1\\
0.122699386503067	0.1\\
0.123456790123457	0.1\\
0.124223602484472	0.1\\
0.125	0.1\\
0.125786163522013	0.1\\
0.126582278481013	0.1\\
0.127388535031847	0.1\\
0.128205128205128	0.1\\
0.129032258064516	0.1\\
0.12987012987013	0.1\\
0.130718954248366	0.1\\
0.131578947368421	0.1\\
0.132450331125828	0.1\\
0.133333333333333	0.1\\
0.134228187919463	0.1\\
0.135135135135135	0.1\\
0.136054421768708	0.1\\
0.136986301369863	0.1\\
0.137931034482759	0.1\\
0.138888888888889	0.1\\
0.13986013986014	0.1\\
0.140845070422535	0.1\\
0.141843971631206	0.1\\
0.142857142857143	0.1\\
0.143884892086331	0.1\\
0.144927536231884	0.1\\
0.145985401459854	0.1\\
0.147058823529412	0.1\\
0.148148148148148	0.1\\
0.149253731343284	0.1\\
0.150375939849624	0.1\\
0.151515151515152	0.1\\
0.152671755725191	0.1\\
0.153846153846154	0.1\\
0.155038759689922	0.1\\
0.15625	0.1\\
0.15748031496063	0.1\\
0.158730158730159	0.1\\
0.16	0.1\\
0.161290322580645	0.1\\
0.16260162601626	0.1\\
0.163934426229508	0.1\\
0.165289256198347	0.1\\
0.166666666666667	0.1\\
0.168067226890756	0.1\\
0.169491525423729	0.1\\
0.170940170940171	0.1\\
0.172413793103448	0.1\\
0.173913043478261	0.1\\
0.175438596491228	0.1\\
0.176991150442478	0.1\\
0.178571428571429	0.1\\
0.18018018018018	0.1\\
0.181818181818182	0.1\\
0.18348623853211	0.1\\
0.185185185185185	0.1\\
0.186915887850467	0.1\\
0.188679245283019	0.1\\
0.19047619047619	0.1\\
0.192307692307692	0.1\\
0.194174757281553	0.1\\
0.196078431372549	0.1\\
0.198019801980198	0.1\\
0.2	0.1\\
0.202020202020202	0.1\\
0.204081632653061	0.1\\
0.206185567010309	0.1\\
0.208333333333333	0.1\\
0.210526315789474	0.1\\
0.212765957446809	0.1\\
0.21505376344086	0.1\\
0.217391304347826	0.1\\
0.21978021978022	0.1\\
0.222222222222222	0.1\\
0.224719101123596	0.1\\
0.227272727272727	0.1\\
0.229885057471264	0.1\\
0.232558139534884	0.1\\
0.235294117647059	0.1\\
0.238095238095238	0.1\\
0.240963855421687	0.1\\
0.24390243902439	0.1\\
0.246913580246914	0.1\\
0.25	0.1\\
0.253164556962025	0.1\\
0.256410256410256	0.1\\
0.25974025974026	0.1\\
0.263157894736842	0.1\\
0.266666666666667	0.1\\
0.27027027027027	0.1\\
0.273972602739726	0.1\\
0.277777777777778	0.1\\
0.28169014084507	0.1\\
0.285714285714286	0.1\\
0.289855072463768	0.1\\
0.294117647058824	0.1\\
0.298507462686567	0.1\\
0.303030303030303	0.1\\
0.307692307692308	0.1\\
0.3125	0.1\\
0.317460317460317	0.1\\
0.32258064516129	0.1\\
0.327868852459016	0.1\\
0.333333333333333	0.1\\
0.338983050847458	0.1\\
0.344827586206897	0.1\\
0.350877192982456	0.1\\
0.357142857142857	0.1\\
0.363636363636364	0.1\\
0.37037037037037	0.1\\
0.377358490566038	0.1\\
0.384615384615385	0.1\\
0.392156862745098	0.1\\
0.4	0.1\\
0.408163265306122	0.1\\
0.416666666666667	0.1\\
0.425531914893617	0.1\\
0.434782608695652	0.1\\
0.444444444444444	0.1\\
0.454545454545455	0.1\\
0.465116279069767	0.1\\
0.476190476190476	0.1\\
0.48780487804878	0.1\\
0.5	0.1\\
};
\addlegendentry{\small Trivial scheme: $\frac{1}{f} H_{\text{min}}$}


\addplot [color=red, line width=1.5pt, mark=o, mark options={red, fill=white}]table[x=coderate,y=OurGenScheme] {fig/data/PC_rate_k20_n400_g2_f10.txt};
\addlegendentry{\small RS-L (Thm.~\ref{thm:PMCrate_LagrangeCoded-DSS})} 


\addplot [color=black, line width=1.5pt, mark=o, mark options={black,fill=white}] table[x=coderate,y=KarpukRaviv] {fig/data/PC_rate_k20_n400_g2_f10.txt}; 
\addlegendentry{\small PPC scheme \cite{RavivKarpuk19_2}}

\addplot [color=blue, line width=1.5pt, mark=diamond*, mark options={solid, blue}] table[x=coderate,y=PCrate_alt_syst] {fig/data/PC_rate_k20_n400_g2_f10.txt}; 
\addlegendentry{\small Sys.~RS-L (Thm.~\ref{thm:RS_PPC_rate})} 

\addplot [color=green, line width=1.5pt, mark=diamond*, mark options={green,fill=white}] table[x=coderate,y=Karpuk] {fig/data/PC_rate_k20_n400_g2_f10.txt}; 
\addlegendentry{\small Sys.~PPC scheme \cite{Karpuk18_1}}


\end{axis}
\end{tikzpicture}%

==> Revision 1/fig/CodedPMC_k2_g2_f2_compare_Sys2.tex <==
% This file was created by matlab2tikz.

\definecolor{mycolor1}{rgb}{0.00000,1.00000,1.00000}%
\definecolor{mycolor2}{rgb}{0.60000,0.00000,0.60000}%
%
\begin{tikzpicture}

\begin{axis}[%
width=4.967in,
height=4.329in,
at={(1.95in,0.779in)},
scale only axis,
every outer x axis line/.append style={black},
every x tick label/.append style={font=\color{black}},
every x tick/.append style={black},
xmin=0.05,
xmax=0.5,
xlabel={Storage code rate $\alpha=k/n$},
every outer y axis line/.append style={black},
every y tick label/.append style={font=\color{black}},
every y tick/.append style={black},
ymin=0.1,
ymax=0.65,
ylabel={PMC rate $\const{R}$},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
xmajorgrids,
ymajorgrids,
grid style={gray,opacity=0.75,dotted},
legend style={legend cell align=left, align=left, draw=white!15!black, fill=white}
]

\addplot [color=mycolor2, dashed, line width=1.5pt, mark=diamond*, mark options={solid, mycolor2}]
table[row sep=crcr]{%
	0.1	0.5\\
	0.105263157894737	0.5\\
	0.111111111111111	0.5\\
	0.117647058823529	0.5\\
	0.125	0.5\\
	0.133333333333333	0.5\\
	0.142857142857143	0.5\\
	0.153846153846154	0.5\\
	0.166666666666667	0.5\\
	0.181818181818182	0.5\\
	0.2	0.5\\
	0.222222222222222	0.5\\
	0.25	0.5\\
	0.285714285714286	0.5\\
	0.333333333333333	0.5\\
	0.4	0.5\\
	0.5	0.5\\
};
\addlegendentry{\small Trivial scheme: $\frac{1}{f} H_{\text{min}}$}


\addplot [color=red, line width=1.5pt, mark=o, mark options={red, fill=white}]
  table[row sep=crcr]{%
0.1	0.567442289345916\\
0.105263157894737	0.562341691586083\\
0.111111111111111	0.556701030927835\\
0.117647058823529	0.550432656504346\\
0.125	0.543429770226457\\
0.133333333333333	0.535561268209083\\
0.142857142857143	0.526665021523951\\
0.153846153846154	0.516539164089487\\
0.166666666666667	0.504930966469428\\
0.181818181818182	0.491523147681875\\
0.2	0.475918522748905\\
0.222222222222222	0.457627118644068\\
0.25	0.436069413392952\\
0.285714285714286	0.410637933983239\\
0.333333333333333	0.380952380952381\\
0.4	0.347801892042293\\
0.5	0.317224287484511\\
};
\addlegendentry{\small RS-L (Thm.~\ref{thm:PMCrate_LagrangeCoded-DSS})} %, $\mu={\mathsf{M}}(f,2)$}



\addplot [color=black, line width=1.5pt, mark=o, mark options={black,fill=white}]
  table[row sep=crcr]{%
0.1	0.566666666666667\\
0.105263157894737	0.56140350877193\\
0.111111111111111	0.555555555555556\\
0.117647058823529	0.549019607843137\\
0.125	0.541666666666667\\
0.133333333333333	0.533333333333333\\
0.142857142857143	0.523809523809524\\
0.153846153846154	0.512820512820513\\
0.166666666666667	0.5\\
0.181818181818182	0.484848484848485\\
0.2	0.466666666666667\\
0.222222222222222	0.444444444444444\\
0.25	0.416666666666667\\
0.285714285714286	0.380952380952381\\
0.333333333333333	0.333333333333333\\
0.4	0.266666666666667\\
0.5	0.166666666666667\\
};
\addlegendentry{\small PPC scheme \cite{RavivKarpuk19_2}}

\addplot [color=blue, line width=1.5pt, mark=diamond*, mark options={solid, blue}]
table[row sep=crcr]{%
	0.1	0.600679056468906\\
	0.105263157894737	0.589448150394178\\
	0.111111111111111	0.589448150394178\\
	0.117647058823529	0.589448150394178\\
	0.125	0.573815644509732\\
	0.133333333333333	0.573815644509732\\
	0.142857142857143	0.573815644509732\\
	0.153846153846154	0.550833781603012\\
	0.166666666666667	0.550833781603012\\
	0.181818181818182	0.550833781603012\\
	0.2	0.514830508474576\\
	0.222222222222222	0.514830508474576\\
	0.25	0.514830508474576\\
	0.285714285714286	0.457142857142857\\
	0.333333333333333	0.457142857142857\\
	0.4	0.457142857142857\\
	0.5	0.372699386503067\\
};

\addlegendentry{\small Sys.~RS-L (Thm.~\ref{thm:RS_PPC_rate})} 

\addplot [color=green, line width=1.5pt, mark=diamond*, mark options={green,fill=white}] 
table[row sep=crcr]{%
	0.1	0.1\\
	0.105263157894737	0.105263157894737\\
	0.111111111111111	0.111111111111111\\
	0.117647058823529	0.117647058823529\\
	0.125	0.125\\
	0.133333333333333	0.133333333333333\\
	0.142857142857143	0.142857142857143\\
	0.153846153846154	0.153846153846154\\
	0.166666666666667	0.166666666666667\\
	0.181818181818182	0.181818181818182\\
	0.2	0.2\\
	0.222222222222222	0.222222222222222\\
	0.25	0.25\\
	0.285714285714286	0.285714285714286\\
	0.333333333333333	0.333333333333333\\
	0.4	0.4\\
	0.5	0.25\\
};
\addlegendentry{\small Sys.~PPC scheme \cite{Karpuk18_1}}

\end{axis}
\end{tikzpicture}%

==> Revision 1/gEX0_axQ-table.tex <==
\begin{table}[htbp!]  
  \centering
  \caption{Sums downloaded for the retrieval of the first linear function evaluation for the 
  example of \cref{sec:PLCex_n2k1f3mu4}.}
  \label{tab:Ex0_axQ-table}
  \vskip -1mm 
  % \Resize[0.7\columnwidth]{
    \begin{IEEEeqnarraybox}[
      \IEEEeqnarraystrutmode
      \IEEEeqnarraystrutsizeadd{3pt}{2pt}]{v/c/v/c/v/c/v}
      \IEEEeqnarrayrulerow\\
      & \text{Database} && 1  && 2 &\\
      \hline\hline
      & 
      && x_{1,1} &&  x_{2,2} &
      \\*\cline{3-7}
      & \multirow{4}{*}{Round $1$}
      && y_{1,1} &&  y_{2,2}  &
      \\
      & && z_{1,1} &&  z_{2,2} &
      \\
      & && w_{1,1}&&  w_{2,2} &
      \\*\hline
      & 
      && x_{3,1}+y_{2,1}   && x_{6,2}+y_{1,2} &
      \\
      & 
      && x_{4,1}+z_{2,1} && x_{7,2}+z_{1,2} &
      \\
      & \multirow{6}{*}{Round $2$}
      && x_{5,1} + w_{2,1} && x_{8,2}+w_{1,2} &
      \\*\cline{3-7}
      & 
      && y_{4,1}+z_{3,1} && y_{7,2}+z_{6,2} &
      \\
      &
      && y_{5,1}+w_{3,1} && y_{8,2}+w_{6,2} &
      \\
      & && z_{5,1}+w_{4,1} && z_{8,2}+w_{7,2} &
      \\*\hline
      & 
      && x_{9,1}+y_{7,1}+z_{6,1}  && x_{12,2}+y_{4,2}+z_{3,2}   &
      \\
      & \multirow{4}{*}{Round $3$}
      && x_{10,1}+y_{8,1}+w_{6,1} && x_{13,2}+y_{5,2}+w_{3,2}   &
      \\
      &
      && x_{11,1}+z_{8,1}+w_{7,1} && x_{14,2}+z_{5,2}+w_{4,2}   &
      \\*\cline{3-7}
      & 
      && y_{11,1}+z_{10,1}+w_{9,1}&& y_{14,2}+z_{13,2}+w_{12,2} &
      \\*\hline
      & \textnormal{Round $4$}
      && x_{15,1}+y_{14,1}+z_{13,1}+w_{12,1} && x_{16,2}+y_{11,2}+z_{10,2} +w_{9,2} &
      \\*\IEEEeqnarrayrulerow
  \end{IEEEeqnarraybox}% }
\end{table}




==> Revision 1/gEX0_table-all.tex <==
\begin{table}[htbp!]  
  \centering
  \caption{Sums downloaded after sign assignment  for the retrieval of the first linear function evaluation for the 
  example of \cref{sec:PLCex_n2k1f3mu4}. For the $1$st database, the sums to be downloaded for $v=3$ are also listed to demonstrate the deterministic sign assignment for a different desired message $\vmat{X}^{(3)}$. The redundant sums are marked in blue.}
  
  \label{tab:answers-table_Ex0}
  \vskip -1mm 
  % \Resize[\columnwidth]{
    \begin{IEEEeqnarraybox}[
      \IEEEeqnarraystrutmode
      \IEEEeqnarraystrutsizeadd{3pt}{2pt}]{v/c/v/c/v/c/v/c/v}
      \IEEEeqnarrayrulerow\\
      & \text{Database} &&  \multicolumn{3}{c}{$1$} && 2 &
      \\*\hline\hline
      & v && 1 && 3 && 1 &\\ \hline
      & 
      && x_{1,1} && x_{1,1} && x_{2,2} &
      \\*\cline{3-9}
      & \multirow{4}{*}{Round $1$}
      && y_{1,1} && y_{1,1} && y_{2,2}  &
      \\
      & && {\b z_{1,1}} && {\b z_{1,1}} && {\b z_{2,2}} &
      \\
      & && {\b w_{1,1}} && {\b w_{1,1}} && {\b w_{2,2}} &
      \\*\hline
      & 
      && x_{3,1}-y_{2,1} && x_{4,1}-y_{3,1} && x_{6,2}-y_{1,2} &
      \\
      & 
      && x_{4,1}-z_{2,1} && x_{2,1}-z_{3,1} && x_{7,2}-z_{1,2} &
      \\
      & \multirow{6}{*}{Round $2$}
      && x_{5,1}-w_{2,1} && x_{5,1}-w_{3,1} && x_{8,2}-w_{1,2} &
      \\*\cline{3-9}
      & 
      && y_{4,1}-z_{3,1} && y_{2,1}-z_{4,1} && y_{7,2}-z_{6,2} &
      \\
      &
      && y_{5,1}-w_{3,1} && y_{5,1}-w_{4,1} && y_{8,2}-w_{6,2} &
      \\
      &
      && {\b z_{5,1}-w_{4,1}} && {\b z_{5,1}-w_{2,1}} && {\b z_{8,2}-w_{7,2}} &
      \\*\hline
      & 
      && x_{9,1}-y_{7,1}+z_{6,1}  && x_{7,1}-y_{6,1}+z_{9,1}  && x_{12,2}-y_{4,2}+z_{3,2}   &
      \\
      & \multirow{4}{*}{Round $3$}
      && x_{10,1}-y_{8,1}+w_{6,1} && x_{11,1}-y_{10,1}+w_{9,1}&& x_{13,2}-y_{5,2}+w_{3,2}   &
      \\
      &
      && x_{11,1}-z_{8,1}+w_{7,1} && -x_{8,1}-z_{10,1}+w_{6,1}&& x_{14,2}-z_{5,2}+w_{4,2}   &
      \\*\cline{3-9}
      & 
      && y_{11,1}-z_{10,1}+w_{9,1}&& -y_{8,1}-z_{11,1}+w_{7,1}&& y_{14,2}-z_{13,2}+w_{12,2} &
      \\*\hline
      & \textnormal{Round $4$}
      && x_{15,1}-y_{14,1}+z_{13,1}-w_{12,1} && x_{14,1}-y_{13,1}+z_{15,1}+w_{12,1} && x_{16,2}-y_{11,2}+z_{10,2}-w_{9,2} &
      \\*\IEEEeqnarrayrulerow
  \end{IEEEeqnarraybox}% }
\end{table}




==> Revision 1/gEX1_axQ-table.tex <==
\begin{table}[htbp!]  
  \centering
  \caption{Auxiliary query sets for each round. Highlighted in red is the {\lin row} % information set
    indicator $u\in[\nu]$ used in determining the indices of the queried symbols. The magenta dashed arrows and the cyan arrows indicate that the \texttt{Exploit-SI} algorithm and the \texttt{M-Sym} algorithm are used, respectively.} 
  \label{tab:axQ-table}
  \vskip -1mm 
  \Resize[0.7\columnwidth]{ % change back to 0.7  the one column version
    \begin{IEEEeqnarraybox}[
      \IEEEeqnarraystrutmode
      \IEEEeqnarraystrutsizeadd{3pt}{2pt}]{v/c/v/c/v/c/v/c/v/c/v}
      \IEEEeqnarrayrulerow\\
      & j && 1  && 2 && 3 && 4\\
      \hline\hline
      & Q^{(1)}_j(a_{1,j},\set{D};1)
      && x_{({\r 1}-1)\cdot 1+1,1} &&  x_{({\r 2}-1)\cdot 1+1,2} && x_{({\r 1}-1)\cdot 1+1,3} && x_{({\r 2}-1)\cdot 1+1,4} &
      \\*\hline
      & \multirow{3}{*}{$Q^{(1)}_j(a_{1,j},\set{U};1)$}
      && y_{({\r 1}-1)\cdot 1+1,1}\tikzmark{y11} &&  y_{({\r 2}-1)\cdot 1+1,2} && y_{({\r 1}-1)\cdot 1+1,3}\tikzmark{y13}
      && y_{({\r 2}-1)\cdot 1+1,4} &
      \\
      & && z_{({\r 1}-1)\cdot 1+1,1}\tikzmark{z11} &&  z_{({\r 2}-1)\cdot 1+1,2} && z_{({\r 1}-1)\cdot 1+1,3}\tikzmark{z13}
      && z_{({\r 2}-1)\cdot 1+1,4} &
      \\
      & && w_{({\r 1}-1)\cdot 1+1,1}\tikzmark{w11} &&  w_{({\r 2}-1)\cdot 1+1,2} && w_{({\r 1}-1)\cdot 1+1,3}\tikzmark{w13}
      && w_{({\r 2}-1)\cdot 1+1,4} &
      \\*\IEEEeqnarrayrulerow
    \end{IEEEeqnarraybox}
}

  (a)
  \\[2mm]
  \Resize[0.8\columnwidth]{ % change back to 0.8 for the one column version
    \begin{IEEEeqnarraybox}[
      \IEEEeqnarraystrutmode
      \IEEEeqnarraystrutsizeadd{3pt}{2pt}]{v/c/v/c/v/c/v/c/v/c/v}
      \IEEEeqnarrayrulerow\\
      & j && 1  && 2 && 3 && 4\\
      \hline\hline
      & \multirow{3}{*}{$Q^{(1)}_j(a_{1,j},\set{D};2)$}
      && x_{1\cdot 2+{\r 1},1}+y_{2,1} &&  x_{1\cdot 2+{\r 2},2}+y_{1,2}\tikzmark{y22} && x_{1\cdot 2+{\r 1},3}+y_{2,3}
      && x_{1\cdot 2+{\r 2},4}+y_{1,4}\tikzmark{y24} &
      \\
      & && x_{2\cdot 2+{\r 1},1}+z_{2,1} && x_{2\cdot 2+{\r 2},2}+z_{1,2}\tikzmark{z22} && x_{2\cdot 2+{\r 1},3}+z_{2,3}
      && x_{2\cdot 2+{\r 2},4}+z_{1,4}\tikzmark{z24} &
      \\
      & && x_{3\cdot 2+{\r 1},1}+w_{2,1} && x_{3\cdot 2+{\r 2},2}+w_{1,2}\tikzmark{w22} && x_{3\cdot 2+{\r 1},3}+w_{2,3}
      && x_{3\cdot 2+{\r 2},4}+w_{1,4}\tikzmark{w24} &
      \\*\hline
      & \multirow{3}{*}{$Q^{(1)}_j(a_{1,j},\set{U};2)$}
      && y_{4+{\r 1},1}+z_{2+{\r 1},1} && y_{4+{\r 2},2}+z_{2+{\r 2},2}\tikzmark{yz22}
      && y_{4+{\r 1},3}+z_{2+{\r 1},3} && y_{4+{\r 2},4}+z_{2+{\r 2},4}\tikzmark{yz24} &
      \\
      & && y_{6+{\r 1},1}+w_{2+{\r 1},1} && y_{6+{\r 2},2}+w_{2+{\r 2},2}\tikzmark{yw22}
      && y_{6+{\r 1},3}+w_{2+{\r 1},3} && y_{6+{\r 2},4}+w_{2+{\r 2},4}\tikzmark{yw24} &
      \\
      & && z_{6+{\r 1},1}+w_{4+{\r 1},1} && z_{6+{\r 2},2}+w_{4+{\r 2},2}\tikzmark{zw22}
      && z_{6+{\r 1},3}+w_{4+{\r 1},3} && z_{6+{\r 2},4}+w_{4+{\r 2},4}\tikzmark{zw24} &
      \\*\IEEEeqnarrayrulerow
    \end{IEEEeqnarraybox}
}

  (b)
  \\[2mm]
  \Resize[\columnwidth]{
    \begin{IEEEeqnarraybox}[
      \IEEEeqnarraystrutmode
      \IEEEeqnarraystrutsizeadd{3pt}{2pt}]{v/c/v/c/v/c/v/c/v/c/v}
      \IEEEeqnarrayrulerow\\
      & j && 1  && 2 && 3 && 4\\
      \hline\hline
      & \multirow{3}{*}{$Q^{(1)}_j(a_{1,j},\set{D};3)$} 
      && x_{4\cdot 2+{\r 1},1}+y_{6,1}+z_{4,1}\tikzmark{yz31} && x_{4\cdot 2+{\r 2},2}+y_{5,2}+z_{3,2}
      && x_{4\cdot 2+{\r 1},3}+y_{6,3}+z_{4,3}\tikzmark{yz33} && x_{4\cdot 2+{\r 2},4}+y_{5,4}+z_{3,4} &
      \\
      & && x_{5\cdot 2+{\r 1},1}+y_{8,1}+w_{4,1}\tikzmark{yw31} && x_{5\cdot 2+{\r 2},2}+y_{7,2}+w_{3,2}
      && x_{5\cdot 2+{\r 1},3}+y_{8,3}+w_{4,3}\tikzmark{yw33} && x_{5\cdot 2+{\r 2},4}+y_{7,4}+w_{3,4} &
       \\
      & && x_{6\cdot 2+{\r 1},1}+z_{8,1}+w_{6,1}\tikzmark{zw31} && x_{6\cdot 2+{\r 2},2}+z_{7,2}+w_{5,2}
      && x_{6\cdot 2+{\r 1},3}+z_{8,3}+w_{6,3}\tikzmark{zw33} && x_{6\cdot 2+{\r 2},4}+z_{7,4}+w_{5,4} &
      \\*\hline
      & Q^{(1)}_j(a_{1,j},\set{U};3)
      && y_{12+{\r 1},1}+z_{10+{\r 1},1}+w_{8+{\r 1},1}\tikzmark{yzw31} && y_{12+{\r 2},2}+z_{10+{\r 2},2}+w_{8+{\r 2},2}
      && y_{12+{\r 1},3}+z_{10+{\r 1},3}+w_{8+{\r 1},3}\tikzmark{yzw33} && y_{12+{\r 2},4}+z_{10+{\r 2},4}+w_{8+{\r 2},4} &
      \\*\IEEEeqnarrayrulerow
    \end{IEEEeqnarraybox}}
  (c)
  \\[2mm]
  \Resize[\columnwidth]{
  	\begin{IEEEeqnarraybox}[
  		\IEEEeqnarraystrutmode
  		\IEEEeqnarraystrutsizeadd{3pt}{2pt}]{v/c/v/c/v/c/v/c/v/c/v}
  		\IEEEeqnarrayrulerow\\
  		& j && 1  && 2 && 3 && 4\\
  		\hline\hline
  		& Q^{(1)}_j(a_{1,j},\set{D};4)
  		&& x_{7\cdot 2+{\r 1},1}+y_{14,1}+z_{12,1}+w_{10,1} && x_{7\cdot 2+{\r 2},2}+y_{13,2}+z_{11,2} +w_{9,2} \tikzmark{yzw42}
  		&& x_{7\cdot 2+{\r 1},3}+y_{14,3}+z_{12,3}+w_{10,3} && \tikzmark{yzw44} x_{7\cdot 2+{\r 2},4}+y_{13,4}+z_{11,4} +w_{9,4}  &
  		\\*\IEEEeqnarrayrulerow
  \end{IEEEeqnarraybox}}
  (d)
  \tikz[overlay,remember picture]{
    \draw[magenta,dashed,>=stealth,->,thick] ($(z11)+(-0.1,-0.80)$) to ($(y22)+(0.65,0.7)$);
    \draw[magenta,dashed,>=stealth,->,thick] ($(z13)+(0.75,-0.80)$) to ($(y22)+(0.65,0.7)$);
    \draw[magenta,dashed,>=stealth,->,thick] ($(z11)+(-0.1,-0.80)$) to ($(y24)+(0.95,0.7)$);
    \draw[magenta,dashed,>=stealth,->,thick] ($(z13)+(0.75,-0.80)$) to ($(y24)+(0.95,0.7)$);
    \path[cyan,>=stealth,->,thick] (w22)+(1.25,0.5) edge [bend left] ($(yz22)+(1.23,0.3)$);
    \path[cyan,>=stealth,->,thick] (w24)+(2.03,0.5) edge [bend left] ($(yz24)+(2.01,0.3)$);
    \draw[magenta,dashed,>=stealth,->,thick] ($(zw22)+(-0.3,-0.2)$) to ($(yz31)+(-0.6,0.2)$);
    \draw[magenta,dashed,>=stealth,->,thick] ($(zw22)+(-0.3,-0.2)$) to ($(yz33)+(-1.2,0.2)$);
    \draw[magenta,dashed,>=stealth,->,thick] ($(zw24)+(-0,-0.2)$) to ($(yz31)+(-0.6,0.2)$);
    \draw[magenta,dashed,>=stealth,->,thick] ($(zw24)+(-0,-0.2)$) to ($(yz33)+(-1.2,0.2)$);
    \path[cyan,>=stealth,->,thick] (zw31)+(-0.01,0.4) edge [bend left] ($(yzw31)+(-0.31,0.2)$);
    \path[cyan,>=stealth,->,thick] (zw33)+(-0.25,0.4) edge [bend left] ($(yzw33)+(-0.55,0.2)$);
    \draw[magenta,dashed,>=stealth,->,thick] ($(yzw31)+(-2.4,-0.2)$) to ($(yzw42)+(-3.3,0.25)$);
    \draw[magenta,dashed,>=stealth,->,thick] ($(yzw33)+(-3.2,-0.2)$) to ($(yzw42)+(-3.3,0.25)$);
    \draw[magenta,dashed,>=stealth,->,thick] ($(yzw31)+(-2.4,-0.2)$) to ($(yzw44)+(-1.35,0.25)$);
    \draw[magenta,dashed,>=stealth,->,thick] ($(yzw33)+(-3.2,-0.2)$) to ($(yzw44)+(-1.35,0.25)$);
  }
  \vskip -2mm 
\end{table}




==> Revision 1/gEX1_table-all.tex <==
\begin{table}[thbp!]
  \centering
  \caption{PLC query sets for $v=1$ after sign assignment for rounds one to four for the $[4,2]$ code of \cref{ex:PLCex_n4k2f4mu4},  $f=4$ messages, and $\mu=4$ candidate linear functions. Red subscripts indicate the indices of the desired linear function evaluations. The redundant queries are marked in blue.}
  \label{tab:answers-table_Ex1}
  \vskip -1mm
  \Resize[\columnwidth]{
    \begin{IEEEeqnarraybox}[
      \IEEEeqnarraystrutmode
      \IEEEeqnarraystrutsizeadd{3pt}{2pt}]{v/c/v/c/v/c/v/c/v/c/v}
      \IEEEeqnarrayrulerow\\
      & j && 1 && 2 && 3 && 4\\
      \hline\hline
      &  Q^{(v)}_j(\set{D};1)
      && x_{{\r 1},1} &&  x_{{\r 2},2} && x_{{\r 1},3} && x_{{\r 2},4} &
      \\*\cline{1-11}      
      & Q^{(v)}_j(\set{U};1)
      && y_{1,1}, {\b z_{1,1},w_{1,1}} &&  y_{2,2},  {\b z_{2,2},  w_{2,2}} && y_{1,3},  {\b z_{1,3},  w_{1,3}} && y_{2,4}, {\b z_{2,4} , w_{2,4}}  &
      \\*\cline{1-11}      
      & \multirow{3}{*}{$Q^{(v)}_j(\set{D};2)$}
      && x_{{\r 3},1}-y_{2,1}&&  x_{{\r 4},2}-y_{1,2} && x_{{\r 3},3}-y_{2,3} && x_{{\r 4},4}-y_{1,4} &
      \\ 
      & 
      && x_{{\r 5},1}-z_{2,1} &&  x_{{\r 6},2}-z_{1,2} && x_{{\r 5},3}-z_{2,3} && x_{{\r 6},4}-z_{1,4} &
      \\ 
      & 
      && x_{{\r 7},1}-w_{2,1}&&  x_{{\r 8},2}-w_{1,2} && x_{{\r 7},3}-w_{2,3} && x_{{\r 8},4}-w_{1,4} &
      \\*\cline{1-11}      
      & \multirow{3}{*}{$Q^{(v)}_j(\set{U};2)$}  
      && y_{5,1}-z_{3,1}&&  y_{6,2}-z_{4,2} && y_{5,3}-z_{3,3} && y_{6,4}-z_{4,4} &
      \\ 
      &  && y_{7,1}-w_{3,1} &&  y_{8,2}-w_{4,2} && y_{7,3}-w_{3,3} && y_{8,4}-w_{4,4} &
      \\ 
      &  && {\b z_{7,1}-w_{5,1}} &&  {\b z_{8,2}-w_{6,2}} && {\b z_{7,3}-w_{5,3}} && {\b z_{8,4}-w_{6,4}} &
      \\*\cline{1-11}      
      & \multirow{3}{*}{$Q^{(v)}_j(\set{D};3)$}
      && x_{{\r 9},1}-y_{6,1}+z_{4,1}  && x_{{\r 10},2}-y_{5,2}+z_{3,2}
      && x_{{\r 9},3}-y_{6,3}+z_{4,3} && x_{{\r 10},4}-y_{5,4}+z_{3,4} &
      \\ 
      & && x_{{\r 11},1}-y_{8,1}+w_{4,1} && x_{{\r 12},2}-y_{7,2}+w_{3,2}
      && x_{{\r 11},3}-y_{8,3}+w_{4,3} && x_{{\r 12},4}-y_{7,4}+w_{3,4} &
      \\ 
      & && x_{{\r 13},1}-z_{8,1}+w_{6,1}  && x_{{\r 14},2}-z_{7,2}+w_{5,2}
      && x_{{\r 13},3}-z_{8,3}+w_{6,3} && x_{{\r 14},4}-z_{7,4}+w_{5,4} &
      \\*\cline{1-11}      
      & Q^{(v)}_j(\set{U};3)
      && y_{13,1}-z_{11,1}+w_{9,1}   && y_{14,2}-z_{12,2}+w_{10,2}
      && y_{13,3}-z_{11,3}+w_{9,3} && y_{14,4}-z_{12,4}+w_{10,4} &   
       \\*\cline{1-11}      
      & Q^{(v)}_j(\set{D};4)
      && x_{{\r 15},1}-y_{14,1}+z_{12,1}-w_{10,1} 
      && x_{{\r 16},2}-y_{13,2}+z_{11,2} -w_{9,2} && x_{{\r 15},3}-y_{14,3}+z_{12,3}-w_{10,3}
      && x_{{\r 16},4}-y_{13,4}+z_{11,4} -w_{9,4}&   
      \\*\IEEEeqnarrayrulerow
    \end{IEEEeqnarraybox}}
    %\vskip -2mm 
\end{table}



==> Revision 1/gEX1_table-all_3.tex <==
\begin{table}[thbp!]
  \centering
  \caption{PLC query sets for $v=3$ after sign assignment for rounds one to four for the $[4,2]$ code of \cref{ex:PLCex_n4k2f4mu4},  $f=4$ messages, and $\mu=4$ candidate linear functions. Red subscripts indicate the indices of the desired linear function evaluations. The redundant queries are marked in blue. }
  \label{tab:answers-table_Ex1_3}
  \vskip -1mm
  \Resize[\columnwidth]{
    \begin{IEEEeqnarraybox}[
      \IEEEeqnarraystrutmode
      \IEEEeqnarraystrutsizeadd{3pt}{2pt}]{v/c/v/c/v/c/v/c/v/c/v}
      \IEEEeqnarrayrulerow\\
      & j && 1 && 2 && 3 && 4\\
      \hline\hline 
      &  Q^{(v)}_j(\set{D};1)
      && {\b z_{{\r 1},1}}&&  {\b z_{{\r 2},2}} && {\b z_{{\r 1},3}} && {\b z_{{\r 2},4}} &
      \\*\cline{1-11}      
      & Q^{(v)}_j(\set{U};1)
      && x_{1,1}, y_{1,1}, {\b w_{1,1}}  &&  x_{2,2},  y_{2,2}, {\b w_{2,2}} && x_{1,3},  y_{1,3}, {\b w_{1,3}} && x_{2,4}, y_{2,4} ,{\b w_{2,4}}  &
      \\*\cline{1-11}      
      & \multirow{3}{*}{$Q^{(v)}_j(\set{D};2)$} 
      && x_{2,1}-z_{{\r 3},1} &&  x_{1,2}-z_{{\r 4},2} && x_{2,3}-z_{{\r 3},3} && x_{1,4}-z_{{\r 4},4} &
      \\ 
      & 
      && y_{2,1}-z_{{\r 5},1} &&  y_{1,2}-z_{{\r 6},2} && y_{2,3}-z_{{\r 5},3} && y_{1,4}-z_{{\r 6},4} &
      \\ 
      & 
      && {\b z_{{\r 7},1}-w_{2,1}} &&  {\b z_{{\r 8},2}-w_{1,2}} && {\b z_{{\r 7},3}-w_{2,3}} && {\b z_{{\r 8},4}-w_{1,4}} &
      \\*\cline{1-11}      
      & \multirow{3}{*}{$Q^{(v)}_j(\set{U};2)$}   
      &&  x_{5,1}-y_{3,1} &&  x_{6,2}-y_{4,2} && x_{5,3}-y_{3,3} && x_{6,4}-y_{4,4} &
      \\ 
      &  &&  x_{7,1}-w_{3,1} &&  x_{8,2}-w_{4,2} && x_{7,3}-w_{3,3} && x_{8,4}-w_{4,4} &
      \\ 
      &  && y_{7,1}-w_{5,1} &&  y_{8,2}-w_{6,2} && y_{7,3}-w_{5,3} &&  y_{8,4}-w_{6,4} &
      \\*\cline{1-11}      
      & \multirow{3}{*}{$Q^{(v)}_j(\set{D};3)$} 
      && x_{6,1}-y_{4,1}+z_{{\r 9},1} && x_{5,2}-y_{3,2}+z_{{\r 10},2}
      && x_{6,3}-y_{4,3}+z_{{\r 9},3} && x_{5,4}-y_{3,4}+z_{{\r10},4} &
      \\ 
      & && -x_{8,1}-z_{{\r 11},1}+w_{4,1} && -x_{7,2}-z_{{\r 12},2}+w_{3,2}
      && -x_{8,3}-z_{{\r 11},3}+w_{4,3} && -x_{7,4}-z_{{\r 12},4}+w_{3,4} &
      \\ 
      & && -y_{8,1}-z_{{\r 13},1}+w_{6,1}  && -y_{7,2}-z_{{\r 14},2}+w_{5,2}
      && -y_{8,3}-z_{{\r 13},3}+w_{6,3} &&- y_{7,4}-z_{{\r 14},4}+w_{5,4} &
      \\*\cline{1-11}      
      & Q^{(v)}_j(\set{U};3) 
      && x_{13,1}-y_{11,1}+w_{9,1}  && x_{14,2}-y_{12,2}+w_{10,2}
      && x_{13,3}-y_{11,3}+w_{9,3} && x_{14,4}-y_{12,4}+w_{10,4} &   
       \\*\cline{1-11}      
      & Q^{(v)}_j(\set{D};4) 
      && x_{14,1}-y_{12,1}+z_{{\r 15},1}+w_{10,1}
      && x_{13,2}-y_{11,2}+z_{{\r 16},2} +w_{9,2} && x_{14,3}-y_{12,3}+z_{{\r 15},3}+w_{10,3}
      && x_{13,4}-y_{11,4}+z_{{\r 16},4} +w_{9,4}&   
      \\*\IEEEeqnarrayrulerow
    \end{IEEEeqnarraybox}}
    %\vskip -2mm 
\end{table}

==> Revision 1/gEX1_table_sortingQ.tex <==
\begin{table}[thbp!]
	\centering
	\caption{PLC query sets for $v=1$ of \cref{ex:PLCex_n4k2f4mu4} after ordering of the queries based on the round and the position of the symbols associated with the desired function evaluation.}
	\label{tab:answers-table_Ex1_sorted}
	\vskip -1mm
	\Resize[\columnwidth]{
		\begin{IEEEeqnarraybox}[
			\IEEEeqnarraystrutmode
			\IEEEeqnarraystrutsizeadd{3pt}{2pt}]{v/c/v/c/v/c/v/c/v/c/v}
			\IEEEeqnarrayrulerow\\
			& (\tau, S, \Delta_{\vmat{U}^{(1)}}(q)) && j=1 && j=2 && j=3 && j=4\\
			\hline\hline
			&  (1, \dots, \dots )
			&& x_{{ 1},1}, y_{1,1}, z_{1,1},w_{1,1} &&  x_{{ 2},2}, y_{2,2},  z_{2,2},  w_{2,2} && x_{{1},3}, y_{1,3},  z_{1,3},  w_{1,3}  && x_{{ 2},4}, y_{2,4},  z_{2,4} , w_{2,4} &
			\\*\cline{1-11}      
			& \multirow{3}{*}{$(2, 1, 1)$}
			&& x_{ 3,1}+y_{2,1}&&  x_{4,2}+y_{1,2} && x_{ 3,3}
			+y_{2,3} && x_{ 4,4}+y_{1,4} &
			\\ 
			& 
			&& x_{ 5,1}+z_{2,1} &&  x_{6,2}+z_{1,2} && x_{ 5,3}+z_{2,3} && x_{6,4}+z_{1,4} &
			\\ 
			& 
			&& x_{ 7,1}+w_{2,1}&&  x_{ 8,2}+w_{1,2} && x_{ 7,3}+w_{2,3} && x_{ 8,4}+w_{1,4} &
			\\*\cline{1-11}      
			& \multirow{3}{*}{$(2, 2, 0)$}  
			&& y_{5,1}+z_{3,1}&&  y_{6,2}+z_{4,2} && y_{5,3}+z_{3,3} && y_{6,4}+z_{4,4} &
			\\ 
			&  && y_{7,1}+w_{3,1} &&  y_{8,2}+w_{4,2} && y_{7,3}+w_{3,3} && y_{8,4}+w_{4,4} &
			\\ 
			&  && { z_{7,1}+w_{5,1}} &&  { z_{8,2}+w_{6,2}} && { z_{7,3}+w_{5,3}} && { z_{8,4}+w_{6,4}} &
			\\*\cline{1-11}      
			& \multirow{3}{*}{$(3, 1, 1)$}
			&& x_{{9},1}+y_{6,1}+z_{4,1}  && x_{{ 10},2}+y_{5,2}+z_{3,2}
			&& x_{{9},3}+y_{6,3}+z_{4,3} && x_{{ 10},4}+y_{5,4}+z_{3,4} &
			\\ 
			& && x_{{11},1}+y_{8,1}+w_{4,1} && x_{{ 12},2}
			+y_{7,2}+w_{3,2}
			&& x_{{11},3}+y_{8,3}+w_{4,3} && x_{{ 12},4}+y_{7,4}+w_{3,4} &
			\\ 
			& && x_{{13},1}+z_{8,1}+w_{6,1}  && x_{{ 14},2}+z_{7,2}+w_{5,2}
			&& x_{{13},3}+z_{8,3}+w_{6,3} && x_{{ 14},4}+z_{7,4}+w_{5,4} &
			\\*\cline{1-11}      
			& (3, 2, 0)
			&& y_{13,1}+z_{11,1}+w_{9,1}   && y_{14,2}+z_{12,2}+w_{10,2}
			&& y_{13,3}+z_{11,3}+w_{9,3} && y_{14,4}+z_{12,4}+w_{10,4} &   
			\\*\cline{1-11}      
			& (4, 1, 1)
			&& x_{{15},1}+y_{14,1}+z_{12,1}+w_{10,1} 
			&& x_{{16},2}+y_{13,2}+z_{11,2} +w_{9,2} && x_{{ 15},3}+y_{14,3}+z_{12,3}+w_{10,3}
			&& x_{{ 16},4}+y_{13,4}+z_{11,4} +w_{9,4}&   
			\\*\IEEEeqnarrayrulerow
	\end{IEEEeqnarraybox}}
	%\vskip -2mm 
\end{table}



==> Revision 1/gEX2_table-all.tex <==
\begin{table}[t]
  \centering
  \caption{The PMC query sets for $v=1$ after sign assignment and removal of redundant queries for a $[4,2]$ RS-coded DSS with Lagrange encoding storing $f=2$ messages, where the $\mu=3$ candidate monomial functions evaluations are $\{\vmat{X}^{(1)}=\vmat{W}^{(1)},\vmat{X}^{(2)}=\vmat{W}^{(2)},\vmat{X}^{(3)}=\vmat{W}^{(1)}\star\vmat{W}^{(2)}\}$. Blue and red subscripts indicate side information exploitation in rounds $\tau=2$ and $\tau=3$, respectively.}
  \label{tab:answers-table}
  \vskip -1mm
  \Resize[\columnwidth]{
    \begin{IEEEeqnarraybox}[
      \IEEEeqnarraystrutmode
      \IEEEeqnarraystrutsizeadd{4pt}{2pt}]{v/c/v/c/v/c/v/c/v/c/v}
      \IEEEeqnarrayrulerow\\
      & j && 1 && 2 && 3 && 4\\
      \hline\hline
      & Q^{(1)}_j(\set{D};1)
      && x_{1:9,1},\, x_{10:18,1},\, x_{19:27,1} &&  x_{1:9,2},\, x_{10:18,2}, \, x_{28:36,2} && x_{1:9,3},\, x_{19:27,3},\, \,x_{28:36,3} && x_{10:18,4},\, x_{19:27,4},\,x_{28:36,4} &
      \\*\cline{1-11}      
      & Q^{(1)}_j(\set{U};1)
      && y_{1:9,1},\, y_{10:18,1},\, y_{19:27,1} &&  y_{1:9,2},\, y_{10:18,2}, \, y_{28:36,2} && y_{1:9,3},\, y_{19:27,3},\, \,y_{28:36,3} && y_{10:18,2},\, y_{19:27,3},\,y_{28:36,4} &
      \\*\cline{1-11}      
      & \multirow{6}{*}{$Q^{(1)}_j(\set{D};2)$}
      && x_{37:39,1}-y_{{\b 28:30},1} &&  x_{37:39,2}-y_{{\b 19:21},2} && x_{37:39,3}-y_{{\b 10:12},3} && x_{43:45,4}-y_{{\b 1:3},4} &
      \\ 
      & 
      && x_{40:42,1}-z_{{\b 28:30},1} &&  x_{40:42,2}-z_{{\b 19:21},2} && x_{40:42,3}-z_{{\b 10:12},3} && x_{46:48,4}-z_{{\b 1:3},4} &
      \\
      &
      && x_{43:45,1}-y_{{\b 31:33},1} &&  x_{43:45,2}-y_{{\b 22:24},2} && x_{49:51,3}-y_{{\b 13:15},3} && x_{49:51,4}-y_{{\b 4:6},4} &
      \\ 
       & 
      && x_{46:48,1}-z_{{\b 31:33},1} &&  x_{46:48,2}-z_{{\b 22:24},2} && x_{52:54,3}-z_{{\b 13:15},3} && x_{52:54,4}-z_{{\b 4:6},4} &
      \\
      &
      && x_{49:51,1}-y_{{\b 34:36},1} &&  x_{55:57,2}-y_{{\b 25:27},2} && x_{55:57,3}-y_{{\b 16:18},3} && x_{55:57,4}-y_{{\b 7:9},4} &
      \\
       & 
      && x_{52:54,1}-z_{{\b 34:36},1} &&  x_{58:60,2}-z_{{\b 25:27},2} && x_{58:60,3}-z_{{\b 16:18},3} && x_{58:60,4}-z_{{\b 7:9},4} &
      \\*\cline{1-11}      
      & \multirow{3}{*}{$Q^{(1)}_j(\set{U};2)$}
      && y_{40:42,1}-z_{37:39,1} &&   y_{40:42,2}-z_{37:39,2} &&  y_{40:42,3}-z_{37:39,3} && y_{46:48,4}-z_{43:45,4} &
      \\
      &
      && y_{46:48,1}-z_{43:45,1} &&  y_{46:48,2}-z_{43:45,2} && y_{52:54,3}-z_{49:51,3} && y_{52:54,4}-z_{49:51,4} &
      \\
      &
      && y_{52:54,1}-z_{49:51,1} &&  y_{58:60,2}-z_{55:57,2} && y_{58:60,3}-z_{55:57,3} && y_{58:60,4}-z_{55:57,4} &
      \\*\cline{1-11}      
      & \multirow{3}{*}{$Q^{(1)}_j(\set{D};3)$}
      && x_{61,1}-y_{{\r  58},1}+z_{{\r  55},1} && x_{61,2}-y_{{\r  52},2}+z_{{\r  49},2}
      && x_{61,3}-y_{{\r  46},3}+z_{{\r  43},3} && x_{62,4}-y_{{\r  40},4}+z_{{\r  37},4} &
      \\
      &
      && x_{62,1}-y_{{\r  59},1}+z_{{\r  56},1} && x_{62,2}-y_{{\r  53},2}+z_{{\r  50},2}
      && x_{63,3}-y_{{\r  47},3}+z_{{\r  44},3} && x_{63,4}-y_{{\r  41},4}+z_{{\r  38},4} &
      \\
      &
      && x_{63,1}-y_{{\r  60},1}+z_{{\r  57},1} && x_{64,2}-y_{{\r  54},2}+z_{{\r  51},2}
      && x_{64,3}-y_{{\r  48},3}+z_{{\r  45},3} && x_{64,4}-y_{{\r  42},4}+z_{{\r  39},4} &
      \\*\IEEEeqnarrayrulerow
    \end{IEEEeqnarraybox}}
    %\vskip -2mm 
\end{table}



==> Revision 1/gEX3_dec-table.tex <==
\begin{table}[h]
  \centering
  \caption{Decoded and computed symbols from the PMC query sets for $v=1$ from \cref{tab:answers-table2}.}
  \label{tab:decoding-table1}
  \vskip -1mm
  \Resize[0.675\columnwidth]{
    \begin{IEEEeqnarraybox}[
      \IEEEeqnarraystrutmode
      \IEEEeqnarraystrutsizeadd{4pt}{2pt}]{v/c/v/c/v/c/v/c/v/c/v}
      \IEEEeqnarrayrulerow\\
      & j && 1 && 2 && 3 && 4\\
      \hline\hline
      & \tilde{Q}^{(1)}_j(\set{D};1)
      && x_{5:8,1} &&  x_{1:4,2} && x_{9:12,3}  && x_{9:12,4} &
      \\*\cline{1-11}      
      & \tilde{Q}^{(1)}_j(\set{U};1)
      && y_{5:8,1},\, z_{5:8,1} && y_{1:4,2},\, z_{1:4,2} &&  y_{9:12,3}, \, z_{9:12,3} &&  y_{9:12,4},\,  z_{9:12,4} &
      \\*\IEEEeqnarrayrulerow
    \end{IEEEeqnarraybox}}
   %\vskip -2mm 
   
(a)
\\[2mm]
\Resize[0.475\columnwidth]{
	\begin{IEEEeqnarraybox}[
		\IEEEeqnarraystrutmode
		\IEEEeqnarraystrutsizeadd{4pt}{2pt}]{v/c/v/c/v/c/v}
		\IEEEeqnarrayrulerow\\
		& j && 1 && 2 \\
		\hline\hline
		& \tilde{Q}^{(1)}_j(\set{D};2)
		&& x_{17:18,1}, \,x_{19:20,1} &&  x_{13:14,2}, \,x_{15:16,2} &% \phantom{x_{21:24,3}}  && \phantom{x_{21:24,4}} &
		\\*\cline{1-7}      
		& \tilde{Q}^{(1)}_j(\set{U};2)
		&&  y_{19:20,1}-z_{17:18,1} &&  y_{15:16,2}-z_{13:14,2} & % \phantom{y_{15:16,2}-z_{13:14,2}} &&  \phantom{y_{15:16,2}-z_{13:14,2}} &
		\\*\IEEEeqnarrayrulerow
\end{IEEEeqnarraybox}}

(b)
\\[2mm]
\Resize[0.5\columnwidth]{
	\begin{IEEEeqnarraybox}[
		\IEEEeqnarraystrutmode
		\IEEEeqnarraystrutsizeadd{4pt}{2pt}]{v/c/v/c/v/c/v}
		\IEEEeqnarrayrulerow\\
		& j && 1 && 2 \\
		\hline\hline
		& \tilde{Q}^{(1)}_j(\set{D};3)
		&& {\b x_{25,1}}, \,x_{27,1} &&  {\b x_{26,2}}, \,x_{27,2} &% \phantom{x_{21:24,3}}  && \phantom{x_{21:24,4}} &
		\\*\cline{1-7}      
		& \tilde{Q}^{(1)}_j(\set{U};3)
		&&  {\b x_{25,1}}+y_{23,1}-z_{21,1} &&  {\b x_{26,2}}+y_{24,2}-z_{22,2} & % \phantom{y_{15:16,2}-z_{13:14,2}} &&  \phantom{y_{15:16,2}-z_{13:14,2}} &
		\\*\IEEEeqnarrayrulerow
\end{IEEEeqnarraybox}}

(c)
\end{table}


==> Revision 1/gEX3_table-all.tex <==
\begin{table}[t]
  \centering
  \caption{PMC query sets for $v=1$ after sign assignment and removal of redundant queries for a $[4,2]$ RS-coded DSS with systematic Lagrange encoding storing $f=2$ messages, where the $\mu=3$ candidate monomial functions evaluations are $\{\vmat{X}^{(1)}=\vmat{W}^{(1)},\vmat{X}^{(2)}=\vmat{W}^{(2)},\vmat{X}^{(3)}=\vmat{W}^{(1)}\star\vmat{W}^{(2)}\}$. Blue and red subscripts indicate side information exploitation in rounds $\tau=2$ and $\tau=3$, respectively.}
  \label{tab:answers-table2}
  \vskip -1mm
  \Resize[0.85\columnwidth]{
    \begin{IEEEeqnarraybox}[
      \IEEEeqnarraystrutmode
      \IEEEeqnarraystrutsizeadd{4pt}{2pt}]{v/c/v/c/v/c/v/c/v/c/v}
      \IEEEeqnarrayrulerow\\
      & j && 1 && 2 && 3 && 4\\
      \hline\hline
      & Q^{(1)}_j(\set{D};1)
      && x_{1:4,1},\, x_{9:12,1} &&  x_{5:8,2},\, x_{9:12,2} && x_{1:4,3}, \,x_{5:8,3} && x_{1:4,4},\, x_{5:8,4} &
      \\*\cline{1-11}      
      & Q^{(1)}_j(\set{U};1)
      && y_{1:4,1},\, y_{9:12,1} &&  y_{5:8,2},\, y_{9:12,2} && y_{1:4,3}, \,y_{5:8,3} && y_{1:4,4},\, y_{5:8,4} &
      \\*\cline{1-11}      
      & \multirow{4}{*}{$Q^{(1)}_j(\set{D};2)$}
      && x_{13:14,1}-y_{{\b 5:6},1} &&  x_{17:18,2}-y_{{\b 1:2},2} && x_{13:14,3}-y_{{\b 9:10},3} && x_{13:14,4}-y_{{\b 9:10},4} &
      \\ 
      & 
      && x_{15:16,1}-z_{{\b 5:6},1} &&  x_{19:20,2}-z_{{\b 1:2},2} && x_{15:16,3}-z_{{\b 9:10},3} && x_{15:16,4}-z_{{\b 9:10},4} &
      \\
      &
      && x_{21:22,1}-y_{{\b 7:8},1} &&  x_{21:22,2}-y_{{\b 3:4},2} && x_{17:18,3}-y_{{\b 11:12},3} && x_{17:18,4}-y_{{\b 11:12},4} &
      \\ 
      & 
      && x_{23:24,1}-z_{{\b 7:8},1} &&  x_{23:24,2}-z_{{\b 3:4},2} && x_{19:20,3}-z_{{\b 11:12},3} && x_{19:20,4}-z_{{\b 11:12},4} &
      \\*\cline{1-11}      
      & \multirow{2}{*}{$Q^{(1)}_j(\set{U};2)$}  
      && y_{15:16,1}-z_{13:14,1} &&  y_{19:20,2}-z_{17:18,2} &&  y_{15:16,3}-z_{13:14,3}&&  y_{15:16,4}-z_{13:14,4} &
      \\
      &
      && y_{23:24,1}-z_{21:22,1} &&  y_{23:24,2}-z_{21:22,2} && y_{19:20,3}-z_{17:18,3} && y_{19:20,4}-z_{17:18,4} &
      \\*\cline{1-11}      
     & \multirow{2}{*}{$Q^{(1)}_j(\set{D};3)$}
      && x_{25,1}-y_{{\r 19},1}+z_{{\r 17},1} && x_{26,2}-y_{{\r 15},2}+z_{{\r 13},2}
      && x_{25,3}-y_{{\r 23},3}+z_{{\r 21},3} && x_{25,4}-y_{{\r 23},4}+z_{{\r 21},4} &
      \\
      &
      && x_{27,1}-y_{{\r 20},1}+z_{{\r 18},1} && x_{27,2}-y_{{\r 16},2}+z_{{\r 14},2}
      && x_{26,3}-y_{{\r 24},3}+z_{{\r 22},3} && x_{26,4}-y_{{\r 24},4}+z_{{\r 22},4} &
      \\*\IEEEeqnarrayrulerow
    \end{IEEEeqnarraybox}}
   %\vskip -2mm 
\end{table}



==> Revision 1/gEXA_axQ-table1.tex <==

\begin{table}[htbp!]  
	\centering
	\caption{Auxiliary query sets for the first round. Highlighted in red is the row % information set
            indicator $u\in[\nu]$ used in determining the indices of the queried symbols. The cyan arrows indicate message symmetry. }
	 \label{tab:axQ-tableA1}
%\Resize[0.6\columnwidth]{
	\begin{IEEEeqnarraybox}[
		\IEEEeqnarraystrutmode
		\IEEEeqnarraystrutsizeadd{3pt}{2pt}]{v/c/v/c/v/c/v/c/v}
		\IEEEeqnarrayrulerow\\
		& j && 1  && 2 && 3\\
		\hline\hline
		& Q^{(1)}_j({\r 1},\set{D};1)
		&& \phantom{x_{1,1},  x_{2,1} ,  x_{3,1} ,  x_{4,1} } && x_{1,2},  x_{2,2} ,  x_{3,2} ,  x_{4,2} \tikzmark{x112e} && \tikzmark{x113b} x_{1,3},  x_{2,3} ,  x_{3,3} ,  x_{4,3} \tikzmark{x113e}&
		\\*\hline
			& \multirow{2}{*}{$Q^{(1)}_j({\r 1},\set{U};1)$}
		&& \phantom{x_{1,1},  x_{2,1} ,  x_{3,1} ,  x_{4,1} } && y_{1,2},  y_{2,2} ,  y_{3,2} ,  y_{4,2}  \tikzmark{y112e} && \tikzmark{y113b} y_{1,3},  y_{2,3} ,  y_{3,3} ,  y_{4,3} \tikzmark{y113e}&
		\\
		& && \phantom{x_{1,1},  x_{2,1} ,  x_{3,1} ,  x_{4,1} } && z_{1,2},  z_{2,2} ,  z_{3,2} ,  z_{4,2}  \tikzmark{z112e}  && z_{1,3},  z_{2,3} ,  z_{3,3} ,  z_{4,3} \tikzmark{z113}&	
		\\*\hline
		& Q^{(1)}_j({\r 2},\set{D};1)
		&& x_{5,1},  x_{6,1} ,  x_{7,1} ,  x_{8,1} \tikzmark{x121e}  && \phantom{x_{9,2},  x_{10,2} ,  x_{11,2} ,  x_{12,2}}  && \tikzmark{x123b} x_{5,3},  x_{6,3} ,  x_{7,3} ,  x_{8,3} \tikzmark{x123e}&
		\\*\hline
		& \multirow{2}{*}{$Q^{(1)}_j({\r 2},\set{U};1)$}
		&&    y_{5,1},  y_{6,1} ,  y_{7,1} ,  y_{8,1} \tikzmark{y121e}  && \phantom{ y_{1,2},  y_{2,2} ,  y_{3,2} ,  y_{4,2} } && \tikzmark{y123b} y_{5,3},  y_{6,3} ,  y_{7,3} ,  y_{8,3} \tikzmark{y123e}&
		\\
		& && z_{5,1},  z_{6,1} ,  z_{7,1} ,  z_{8,1} \tikzmark{z121e} &&\phantom{ z_{1,2},  z_{2,2} ,  z_{3,2} ,  z_{4,2}}  && z_{5,3},  z_{6,3} ,  z_{7,3} ,  z_{8,3} \tikzmark{z123e} &	
		\\*\hline
		& Q^{(1)}_j({\r 3},\set{D};1)
		&& x_{9,1},  x_{10,1} ,  x_{11,1} ,  x_{12,1} \, \tikzmark{x131e} && \tikzmark{x132b}\, x_{9,2},  x_{10,2} ,  x_{11,2} ,  x_{12,2}  \tikzmark{x132e}&& \phantom{x_{1,3},  x_{2,3} ,  x_{3,3} ,  x_{4,3}}&
		\\*\hline
		& \multirow{2}{*}{$Q^{(1)}_j({\r 3},\set{U};1)$}
		&&     y_{9,1},  y_{10,1} ,  y_{11,1} ,  y_{12,1}   \tikzmark{y131e} && \tikzmark{y132b} \, y_{9,2},  y_{10,2} ,  y_{11,2} ,  y_{12,2} \, \tikzmark{y132e}  && \phantom{y_{9,3},  y_{10,3} ,  y_{11,3} ,  y_{12,3} }&
		\\
		& && z_{9,1},  z_{10,1} ,  z_{11,1} ,  z_{12,1} \tikzmark{z131e}  && \tikzmark{z132b} z_{9,2},  z_{10,2} ,  z_{11,2} ,  z_{12,2} \, \tikzmark{z132e}  && \phantom{z_{1,3},  z_{2,3} ,  z_{3,3} ,  z_{4,3}}&	
		\\*\IEEEeqnarrayrulerow
\end{IEEEeqnarraybox}
% }   naming of tikzmark follows {x,y,z}+ {\tau} + {u}+ {j} +{b,e} for begning or end of the cell
 \tikz[overlay,remember picture]{
	\path[cyan,>=stealth,->,thick] (x112e)+(0.2,0) edge [bend left] ($(y112e)+(0.2,-0.3)$);
	\path[cyan,>=stealth,->,thick] (x113e)+(0.2,0) edge [bend left] ($(y113e)+(0.2,-0.3)$);
	\path[cyan,>=stealth,->,thick] (x121e)+(0.2,0) edge [bend left] ($(y121e)+(0.2,-0.3)$);
	\path[cyan,>=stealth,->,thick] (x123e)+(0.2,0) edge [bend left] ($(y123e)+(0.2,-0.3)$);
	\path[cyan,>=stealth,->,thick] (x131e)+(0.05,0) edge [bend left] ($(y131e)+(0.05,-0.3)$);
	\path[cyan,>=stealth,->,thick] (x132e)+(0.05,0) edge [bend left] ($(y132e)+(0.05,-0.3)$);
}
\end{table}


==> Revision 1/gEXA_axQ-table2.tex <==
\begin{table}[htbp!]  
	\centering
	\caption{Initial auxiliary query sets for the second round. Highlighted in red is the row % information set
            indicator $u\in[\nu]$ used in determining the indices of the queried symbols.}
	 \label{tab:axQ-tableA2}
%\Resize[0.6\columnwidth]{
	\begin{IEEEeqnarraybox}[
		\IEEEeqnarraystrutmode
		\IEEEeqnarraystrutsizeadd{3pt}{2pt}]{v/c/v/c/v/c/v/c/v}
		\IEEEeqnarrayrulerow\\
		& j && 1  && 2 && 3\\
		\hline\hline
			& \multirow{2}{*}{$Q^{(1)}_j({\r 1},\set{D};2)$}
		&& \phantom{x_{1,1},  x_{2,1} ,  x_{3,1} } && x_{4\cdot3+{\r 1},2},  && x_{4\cdot3+{\r 1},3}, &
		\\
		& && \phantom{x_{16,1},  x_{19,1} ,  x_{22,1}  } && x_{16,2},  x_{19,2} ,  x_{22,2}  && x_{16,3},  x_{19,3} ,  x_{22,3}  &	
		\\*\hline
		& \multirow{2}{*}{$Q^{(1)}_j({\r 2},\set{D};2)$}
		&&    x_{4\cdot3+{\r 2},1},  && \phantom{ y_{1,2},  y_{2,2} ,  y_{3,2}} && x_{4\cdot3+{\r 2},3}  &
		\\
		& && x_{17,1},  x_{20,1} ,  x_{23,1}  &&\phantom{ z_{1,2},  z_{2,2} ,  z_{3,2} }  && x_{17,3},  x_{20,3} ,  x_{23,3} &	
		\\*\hline
		& \multirow{2}{*}{$Q^{(1)}_j({\r 3},\set{D};2)$}
		&&     x_{4\cdot3+{\r 3},1}, &&  x_{4\cdot3+{\r 3},2},   && \phantom{y_{9,3},  y_{10,3} ,  y_{11,3} }&
		\\
		& && x_{18,1},  x_{21,1} ,  x_{24,1} && x_{18,2},  x_{21,2} ,  x_{24,2}   && \phantom{x_{1,3},  x_{21,3} ,  x_{24,3}}&	
		\\*\IEEEeqnarrayrulerow
\end{IEEEeqnarraybox}
% }   naming of tikzmark follows {x,y,z}+ {\tau} + {u}+ {j} +{b,e} for begning or end of the cell
 %\tikz[overlay,remember picture]{
%	\draw[magenta,dashed,>=stealth,<->,thick] ($(x112e)+(0.1,0)$) to ($(x113b)+(-0.1,0)$);
%	\draw[magenta,dashed,>=stealth,<->,thick] ($(y112e)+(0.1,-0.25)$) to ($(y113b)+(-0.1,-0.25)$);
%	\path[cyan,>=stealth,->,thick] (x112e)+(0.2,0) edge [bend left] ($(y112e)+(0.2,-0.3)$);
%	\path[cyan,>=stealth,->,thick] (x113e)+(0.2,0) edge [bend left] ($(y113e)+(0.2,-0.3)$);
	%
%	\draw[magenta,dashed,>=stealth,<->,thick] ($(x121e)+(0.1,0)$) to ($(x123b)+(-0.1,0)$);
%	\draw[magenta,dashed,>=stealth,<->,thick] ($(y121e)+(0.1,-0.25)$) to ($(y123b)+(-0.1,-0.25)$);
%	\path[cyan,>=stealth,->,thick] (x121e)+(0.2,0) edge [bend left] ($(y121e)+(0.2,-0.3)$);
%	\path[cyan,>=stealth,->,thick] (x123e)+(0.2,0) edge [bend left] ($(y123e)+(0.2,-0.3)$);
	%
%	\draw[magenta,dashed,>=stealth,<->,thick] ($(x131e)+(-0.01,0)$) to ($(x132b)+(0,0)$);
%	\draw[magenta,dashed,>=stealth,<->,thick] ($(y131e)+(-0.01,-0.25)$) to ($(y132b)+(0,-0.25)$);
%	\path[cyan,>=stealth,->,thick] (x131e)+(0.05,0) edge [bend left] ($(y131e)+(0.05,-0.3)$);
%	\path[cyan,>=stealth,->,thick] (x132e)+(0.05,0) edge [bend left] ($(y132e)+(0.05,-0.3)$);
%}
\end{table}


==> Revision 1/gEXA_axQ-table3.tex <==
\begin{table}[htbp!]  
	\centering
	\caption{Side information generation and exploitation. (a) shows the side information generated by the \texttt{Exploit-SI} algorithm from the auxiliary query sets of the first round. The generated side information shown in (a) is exploited in forming $\tau$-sums of the final auxiliary query sets of the second round shown in (b). The cyan arrows indicate that the \texttt{M-Sym} algorithm is used. Finally, highlighted in red is the row % information set
            indicator $u\in[\nu]$ used in determining the indices of the queried symbols. 
	}
	 \label{tab:axQ-tableA3}
%\Resize[0.6\columnwidth]{
	\begin{IEEEeqnarraybox}[
		\IEEEeqnarraystrutmode
		\IEEEeqnarraystrutsizeadd{3pt}{2pt}]{v/c/v/c/v/c/v/c/v}
		\IEEEeqnarrayrulerow\\
		& j && 1  && 2 && 3\\
		\hline\hline
			& \multirow{2}{*}{$Q^{(1)}_j({\r 1},\set{U};1)$}
		&&  y_{1,1},  y_{2,1} ,  y_{3,1} ,  y_{4,1}  && \phantom{y_{1,2},  y_{2,2} ,  y_{3,2} ,  y_{4,2}}  && \phantom{ y_{1,3},  y_{2,3} ,  y_{3,3} ,  y_{4,3} }&
		\\
		& && z_{1,1},  z_{2,1} ,  z_{3,1} ,  z_{4,1}  &&  \phantom{z_{1,2},  z_{2,2} ,  z_{3,2} ,  z_{4,2}}   && \phantom{z_{1,3},  z_{2,3} ,  z_{3,3} ,  z_{4,3}}&	
		\\*\hline
		& \multirow{2}{*}{$Q^{(1)}_j({\r 2},\set{U};1)$}
		&&    \phantom{y_{5,1},  y_{6,1} ,  y_{7,1} ,  y_{8,1}}  && y_{5,2},  y_{6,2} ,  y_{7,2} ,  y_{8,2} && \phantom{ y_{5,3},  y_{6,3} ,  y_{7,3} ,  y_{8,3} }&
		\\
		& && \phantom{z_{5,1},  z_{6,1} ,  z_{7,1} ,  z_{8,1}} &&z_{5,2},  z_{6,2} ,  z_{7,2} ,  z_{8,2} && \phantom{ z_{5,3},  z_{6,3} ,  z_{7,3} ,  z_{8,3} } &	
		\\*\hline
		& \multirow{2}{*}{$Q^{(1)}_j({\r 3},\set{U};1)$}
		&&     \phantom{y_{9,1},  y_{10,1} ,  y_{11,1} ,  y_{12,1}}   &&  \phantom{ y_{9,2},  y_{10,2} ,  y_{11,2} ,  y_{12,2} } && y_{9,3},  y_{10,3} ,  y_{11,3} ,  y_{12,3} &
		\\
		& && \phantom{z_{9,1},  z_{10,1} ,  z_{11,1} ,  z_{12,1} }  && \phantom{ z_{9,2},  z_{10,2} ,  z_{11,2} ,  z_{12,2}} && z_{9,3},  z_{10,3} ,  z_{11,3} ,  z_{12,3}&	
		\\*\IEEEeqnarrayrulerow
\end{IEEEeqnarraybox}

 (a)
\\[2mm]

	\begin{IEEEeqnarraybox}[
	\IEEEeqnarraystrutmode
	\IEEEeqnarraystrutsizeadd{3pt}{2pt}]{v/c/v/c/v/c/v/c/v}
	\IEEEeqnarrayrulerow\\
	& j && 1  && 2 && 3\\
	\hline\hline
	& \multirow{4}{*}{$Q^{(1)}_j({\r 1},\set{D};2)$}
	&& \phantom{y_{1,1},  y_{2,1} ,  y_{3,1} ,  y_{4,1}} && x_{13,2} + y_{5,2}  && x_{13,3}+ y_{9,3} &
		\\
	& && \phantom{x_{16,2} + z_{5,2}  } && x_{16,2} + z_{5,2} && x_{16,3} +z_{9,3}   &	
		\\
	& && \phantom{x_{19,2} + y_{7,2} } && x_{19,2} + y_{7,2} &&  x_{19,3} +y_{11,3}  &	
		\\
	& && \phantom{x_{22,2} +  z_{7,2}  } && x_{22,2} +  z_{7,2}  \tikzmark{x212e}&& x_{22,3} +z_{11,3} \tikzmark{x213e}  &	
	\\*\hline
	& \multirow{2}{*}{$Q^{(1)}_j({\r 1},\set{U};2)$}
		&& \phantom{y_{17,1}+z_{ 14,1}} && y_{16,2} + z_{13,2} \tikzmark{y212e} && y_{16,3} +z_{13,3}  \tikzmark{y213e}  &	
	\\
	& && \phantom{y_{23,1}+z_{ 20,1}}&& y_{22,2} +  z_{19,2}  \tikzmark{z212e}  && y_{22,3} +z_{19,3} \tikzmark{z213} &	
	\\*\hline
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	& \multirow{4}{*}{$Q^{(1)}_j({\r 2},\set{D};2)$}
	&&    x_{14,1}+y_{ 1,1}  && \phantom{ y_{5,2},  y_{6,2} ,  y_{7,2} ,  y_{8,2}} && x_{14,3}+y_{10,3} &
	\\
	& && x_{17,1}+z_{ 1,1}  && \phantom{ x_{17,3}+z_{11,3}}  && x_{17,3}+z_{10,3} &	
	\\
	& && x_{20,1}+y_{ 3,1} && \phantom{ x_{20,3} +y_{12,3} }  && x_{20,3} +y_{12,3} &	
	\\
	& &&  x_{23,1}+z_{ 3,1} \tikzmark{x221e} &&\phantom{  x_{23,3}+z_{12,3}}  &&  x_{23,3}+z_{12,3} \tikzmark{x223e}&	
	\\*\hline
		& \multirow{2}{*}{$Q^{(1)}_j({\r 2},\set{U};2)$}
	&& y_{17,1}+z_{ 14,1} \tikzmark{y221e} && \phantom{y_{16,2} + z_{13,2} } && y_{17,3}+z_{14,3}  \tikzmark{y223e}&	
	\\
	& && y_{23,1}+z_{ 20,1}  \tikzmark{z221e}  && \phantom{y_{22,2} +  z_{19,2} }  && y_{23,3}+z_{20,3}\tikzmark{z223e} &	
	\\*\hline
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	& \multirow{4}{*}{$Q^{(1)}_j({\r 3},\set{D};2)$}
	&&     x_{15,1}+y_{ 2,1}  &&  x_{15,2}+y_{6,2}  && \phantom{y_{9,2},  y_{10,2} ,  y_{11,2} ,  y_{12,2}}&
	\\
	& && x_{18,1}+z_{ 2,1}  && x_{18,2}+z_{ 6,2} && \phantom{x_{1,3},  x_{21,3} ,  x_{24,3}}&	
		\\
	& && x_{21,1}+y_{ 4,1} && x_{21,2}+y_{ 8,2}   && \phantom{x_{1,3},  x_{21,3} ,  x_{24,3}}&	
		\\
	& &&  x_{24,1}+z_{ 4,1} \tikzmark{x231e} &&   x_{24,2}+z_{8 ,2}   \tikzmark{x232e} && \phantom{x_{1,3},  x_{21,3} ,  x_{24,3}}&	
	\\*\hline
	& \multirow{2}{*}{$Q^{(1)}_j({\r 3},\set{U};2)$}
	&& y_{18,1}+z_{ 15,1} \tikzmark{y231e}  && y_{18,2}+z_{ 15,2} \tikzmark{y232e}  && \phantom{y_{17,3}+z_{14,3}} &	
	\\	
	& &&  y_{24,1}+z_{ 21,1} \tikzmark{z231e}  &&y_{24,2}+z_{21 ,2} \tikzmark{z232e}    && \phantom{ y_{23,3}+z_{20,3} }&	
	\\*\IEEEeqnarrayrulerow
\end{IEEEeqnarraybox}

(b)

% }   naming of tikzmark follows {x,y,z}+ {\tau} + {u}+ {j} +{b,e} for begning or end of the cell
 \tikz[overlay,remember picture]{
%	\draw[magenta,dashed,>=stealth,<->,thick] ($(x112e)+(0.1,0)$) to ($(x113b)+(-0.1,0)$);
%	\draw[magenta,dashed,>=stealth,<->,thick] ($(y112e)+(0.1,-0.25)$) to ($(y113b)+(-0.1,-0.25)$);
	\path[cyan,>=stealth,->,thick] (x212e)+(0.2,0) edge [bend left] ($(y212e)+(0.2,-0.3)$);
	\path[cyan,>=stealth,->,thick] (x213e)+(0.2,0) edge [bend left] ($(y213e)+(0.2,-0.3)$);
	%
%	\draw[magenta,dashed,>=stealth,<->,thick] ($(x121e)+(0.1,0)$) to ($(x123b)+(-0.1,0)$);
%	\draw[magenta,dashed,>=stealth,<->,thick] ($(y121e)+(0.1,-0.25)$) to ($(y123b)+(-0.1,-0.25)$);
	\path[cyan,>=stealth,->,thick] (x221e)+(0.2,0) edge [bend left] ($(y221e)+(0.2,-0.3)$);
	\path[cyan,>=stealth,->,thick] (x223e)+(0.2,0) edge [bend left] ($(y223e)+(0.2,-0.3)$);
	%
%	\draw[magenta,dashed,>=stealth,<->,thick] ($(x131e)+(-0.01,0)$) to ($(x132b)+(0,0)$);
%	\draw[magenta,dashed,>=stealth,<->,thick] ($(y131e)+(-0.01,-0.25)$) to ($(y132b)+(0,-0.25)$);
	\path[cyan,>=stealth,->,thick] (x231e)+(0.05,0) edge [bend left] ($(y231e)+(0.05,-0.3)$);
	\path[cyan,>=stealth,->,thick] (x232e)+(0.05,0) edge [bend left] ($(y232e)+(0.05,-0.3)$);
}
\end{table}


==> Revision 1/gEXA_axQ-table4.tex <==
\begin{table}[htbp!]  
	\centering
	\caption{Generic PC query sets for $v=1$ for the generic PC achievable rate matrix $\mat{\Lambda}^{\textnormal{PC}}_{2,3}$ of \cref{ex:MDSCapCodeex_n3k2}, $f=2$ messages, and $\mu=3$ candidate functions.} 
	 \label{tab:axQ-tableA4}
%\Resize[0.6\columnwidth]{
	\begin{IEEEeqnarraybox}[
		\IEEEeqnarraystrutmode
		\IEEEeqnarraystrutsizeadd{3pt}{2pt}]{v/c/v/c/v/c/v/c/v}
		\IEEEeqnarrayrulerow\\
		& j && 1  && 2 && 3\\
		\hline\hline
			& \multirow{2}{*}{$Q^{(1)}_j(\set{D};1)$}
		&& x_{5,1},  x_{6,1} ,  x_{7,1} ,  x_{8,1} \tikzmark{x121e} && x_{1,2},  x_{2,2} ,  x_{3,2} ,  x_{4,2} \tikzmark{x112e} &&  \tikzmark{x113b} x_{1,3},  x_{2,3} ,  x_{3,3} ,  x_{4,3} \tikzmark{x113e}&
		\\ \cline{3-9}
		& &&  x_{9,1},  x_{10,1} ,  x_{11,1} ,  x_{12,1} \, \tikzmark{x131e}  && \tikzmark{x132b}\, x_{9,2},  x_{10,2} ,  x_{11,2} ,  x_{12,2} \tikzmark{x132e} &&\tikzmark{x123b} x_{5,3},  x_{6,3} ,  x_{7,3} ,  x_{8,3} \tikzmark{x123e}&
		\\*\hline
			& \multirow{4}{*}{$Q^{(1)}_j(\set{U};1)$}
		&& y_{5,1},  y_{6,1} ,  y_{7,1} ,  y_{8,1} \tikzmark{y121e} && y_{1,2},  y_{2,2} ,  y_{3,2} ,  y_{4,2}  \tikzmark{y112e} && \tikzmark{y113b} y_{1,3},  y_{2,3} ,  y_{3,3} ,  y_{4,3} \tikzmark{y113e}&
		\\
		& && z_{5,1},  z_{6,1} ,  z_{7,1} ,  z_{8,1} \tikzmark{z121e}&& z_{1,2},  z_{2,2} ,  z_{3,2} ,  z_{4,2}  \tikzmark{z112e}  && z_{1,3},  z_{2,3} ,  z_{3,3} ,  z_{4,3} \tikzmark{z113}&
		\\ \cline{3-9}
		&  &&  y_{9,1},  y_{10,1} ,  y_{11,1} ,  y_{12,1}   \tikzmark{y131e} && \tikzmark{y132b} \, y_{9,2},  y_{10,2} ,  y_{11,2} ,  y_{12,2} \, \tikzmark{y132e} && \tikzmark{y123b} y_{5,3},  y_{6,3} ,  y_{7,3} ,  y_{8,3} \tikzmark{y123e}&
		\\
		& &&z_{9,1},  z_{10,1} ,  z_{11,1} ,  z_{12,1} \tikzmark{z131e}  && \tikzmark{z132b} z_{9,2},  z_{10,2} ,  z_{11,2} ,  z_{12,2} \, \tikzmark{z132e}   &&  z_{5,3},  z_{6,3} ,  z_{7,3} ,  z_{8,3} \tikzmark{z123e} &	
		\\*\hline
			& \multirow{8}{*}{$Q^{(1)}_j(\set{D};2)$}
		&& x_{14,1}+y_{ 1,1} && x_{13,2} + y_{5,2}  && x_{13,3}+ y_{9,3} &
		\\
		& && x_{17,1}+z_{ 1,1} && x_{16,2} + z_{5,2} && x_{16,3} +z_{9,3}    &	
		\\
		& && x_{20,1}+y_{ 3,1} && x_{19,2} + y_{7,2} &&  x_{19,3} +y_{11,3}  &	
		\\
		& && x_{23,1}+z_{ 3,1} && x_{22,2} +  z_{7,2} && x_{22,3} +z_{11,3}  &	
		\\\cline{3-9}
		& &&     x_{15,1}+y_{ 2,1}   &&  x_{15,2}+y_{6,2} && x_{14,3}+y_{10,3} &
		\\
		& && x_{18,1}+z_{ 2,1} && x_{18,2}+z_{ 6,2} && x_{17,3}+z_{10,3} &	
		\\
		& && x_{21,1}+y_{ 4,1} && x_{21,2}+y_{ 8,2}  && x_{20,3} +y_{12,3} &	
		\\
		& &&  x_{24,1}+z_{ 4,1}&&x_{24,2}+z_{8 ,2}   &&  x_{23,3}+z_{12,3} &	
		\\*\hline
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		& \multirow{4}{*}{$Q^{(1)}_j(\set{U};2)$}
		&& y_{17,1}+z_{ 14,1} && y_{16,2} + z_{13,2} && y_{16,3} +z_{13,3}    &	
		\\
		& && y_{23,1}+z_{ 20,1} && y_{22,2} +  z_{19,2} && y_{22,3} +z_{19,3}  &	
		\\\cline{3-9}
		& && y_{18,1}+z_{ 15,1} && y_{18,2}+z_{ 15,2} && y_{17,3}+z_{14,3} &	
		\\	
		& &&  y_{24,1}+z_{ 21,1}&&y_{24,2}+z_{21 ,2}   &&  y_{23,3}+z_{20,3} &
		\\*\hline	
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		& \multirow{2}{*}{$Q^{(1)}_j(\set{D};3)$}
		 && x_{26 ,1}+y_{16,1}+z_{ 13,1} &&x_{25,2} +y_{17,2} + z_{14,2} &&x_{ 25,3}+ y_{18,3} +z_{15,3}    &		
		\\\cline{3-9}
		& && x_{ 27,1}+y_{22,1}+z_{ 19,1} && x_{27,2} + y_{23,2}+z_{ 20,2} && x_{ 26,3}+y_{24,3}+z_{21,3} &		
		\\*\IEEEeqnarrayrulerow
\end{IEEEeqnarraybox}
% }   naming of tikzmark follows {x,y,z}+ {\tau} + {u}+ {j} +{b,e} for begning or end of the cell
% \tikz[overlay,remember picture]{
%	\draw[magenta,dashed,>=stealth,<->,thick] ($(x112e)+(0.1,0)$) to ($(x113b)+(-0.1,0)$);
%	\draw[magenta,dashed,>=stealth,<->,thick] ($(y112e)+(0.1,-0.25)$) to ($(y113b)+(-0.1,-0.25)$);
%	\path[cyan,>=stealth,->,thick] (x112e)+(0.2,0) edge [bend left] ($(y112e)+(0.2,-0.3)$);
%	\path[cyan,>=stealth,->,thick] (x113e)+(0.2,0) edge [bend left] ($(y113e)+(0.2,-0.3)$);
	%
%	\draw[magenta,dashed,>=stealth,<->,thick] ($(x121e)+(0.1,0)$) to ($(x123b)+(-0.1,0)$);
%	\draw[magenta,dashed,>=stealth,<->,thick] ($(y121e)+(0.1,-0.25)$) to ($(y123b)+(-0.1,-0.25)$);
%	\path[cyan,>=stealth,->,thick] (x121e)+(0.2,0) edge [bend left] ($(y121e)+(0.2,-0.3)$);
%	\path[cyan,>=stealth,->,thick] (x123e)+(0.2,0) edge [bend left] ($(y123e)+(0.2,-0.3)$);
	%
%	\draw[magenta,dashed,>=stealth,<->,thick] ($(x131e)+(-0.01,0)$) to ($(x132b)+(0,0)$);
%	\draw[magenta,dashed,>=stealth,<->,thick] ($(y131e)+(-0.01,-0.25)$) to ($(y132b)+(0,-0.25)$);
%	\path[cyan,>=stealth,->,thick] (x131e)+(0.05,0) edge [bend left] ($(y131e)+(0.05,-0.3)$);
%	\path[cyan,>=stealth,->,thick] (x132e)+(0.05,0) edge [bend left] ($(y132e)+(0.05,-0.3)$);
%}
\end{table}

==> gEX0_axQ-table.tex <==
\begin{table}[htbp!]  
  \centering
  \caption{Sums downloaded for the retrieval of the first linear function evaluation for the 
  example of \cref{sec:PLCex_n2k1f3mu4}.}
  \label{tab:Ex0_axQ-table}
  \vskip -1mm 
  % \Resize[0.7\columnwidth]{
    \begin{IEEEeqnarraybox}[
      \IEEEeqnarraystrutmode
      \IEEEeqnarraystrutsizeadd{3pt}{2pt}]{v/c/v/c/v/c/v}
      \IEEEeqnarrayrulerow\\
      & \text{Database} && 1  && 2 &\\
      \hline\hline
      & 
      && x_{1,1} &&  x_{2,2} &
      \\*\cline{3-7}
      & \multirow{4}{*}{Round $1$}
      && y_{1,1} &&  y_{2,2}  &
      \\
      & && z_{1,1} &&  z_{2,2} &
      \\
      & && w_{1,1}&&  w_{2,2} &
      \\*\hline
      & 
      && x_{3,1}+y_{2,1}   && x_{6,2}+y_{1,2} &
      \\
      & 
      && x_{4,1}+z_{2,1} && x_{7,2}+z_{1,2} &
      \\
      & \multirow{6}{*}{Round $2$}
      && x_{5,1} + w_{2,1} && x_{8,2}+w_{1,2} &
      \\*\cline{3-7}
      & 
      && y_{4,1}+z_{3,1} && y_{7,2}+z_{6,2} &
      \\
      &
      && y_{5,1}+w_{3,1} && y_{8,2}+w_{6,2} &
      \\
      & && z_{5,1}+w_{4,1} && z_{8,2}+w_{7,2} &
      \\*\hline
      & 
      && x_{9,1}+y_{7,1}+z_{6,1}  && x_{12,2}+y_{4,2}+z_{3,2}   &
      \\
      & \multirow{4}{*}{Round $3$}
      && x_{10,1}+y_{8,1}+w_{6,1} && x_{13,2}+y_{5,2}+w_{3,2}   &
      \\
      &
      && x_{11,1}+z_{8,1}+w_{7,1} && x_{14,2}+z_{5,2}+w_{4,2}   &
      \\*\cline{3-7}
      & 
      && y_{11,1}+z_{10,1}+w_{9,1}&& y_{14,2}+z_{13,2}+w_{12,2} &
      \\*\hline
      & \textnormal{Round $4$}
      && x_{15,1}+y_{14,1}+z_{13,1}+w_{12,1} && x_{16,2}+y_{11,2}+z_{10,2} +w_{9,2} &
      \\*\IEEEeqnarrayrulerow
  \end{IEEEeqnarraybox}% }
\end{table}




==> gEX0_table-all.tex <==
\begin{table}[htbp!]  
  \centering
  \caption{Sums downloaded after sign assignment  for the retrieval of the first linear function evaluation for the 
  example of \cref{sec:PLCex_n2k1f3mu4}. For the $1$st database, the sums to be downloaded for $v=3$ are also listed to demonstrate the deterministic sign assignment for a different desired message $\vmat{X}^{(3)}$. The redundant sums are marked in blue.}
  
  \label{tab:answers-table_Ex0}
  \vskip -1mm 
  % \Resize[\columnwidth]{
    \begin{IEEEeqnarraybox}[
      \IEEEeqnarraystrutmode
      \IEEEeqnarraystrutsizeadd{3pt}{2pt}]{v/c/v/c/v/c/v/c/v}
      \IEEEeqnarrayrulerow\\
      & \text{Database} &&  \multicolumn{3}{c}{$1$} && 2 &
      \\*\hline\hline
      & v && 1 && 3 && 1 &\\ \hline
      & 
      && x_{1,1} && x_{1,1} && x_{2,2} &
      \\*\cline{3-9}
      & \multirow{4}{*}{Round $1$}
      && y_{1,1} && y_{1,1} && y_{2,2}  &
      \\
      & && {\b z_{1,1}} && {\b z_{1,1}} && {\b z_{2,2}} &
      \\
      & && {\b w_{1,1}} && {\b w_{1,1}} && {\b w_{2,2}} &
      \\*\hline
      & 
      && x_{3,1}-y_{2,1} && x_{4,1}-y_{3,1} && x_{6,2}-y_{1,2} &
      \\
      & 
      && x_{4,1}-z_{2,1} && x_{2,1}-z_{3,1} && x_{7,2}-z_{1,2} &
      \\
      & \multirow{6}{*}{Round $2$}
      && x_{5,1}-w_{2,1} && x_{5,1}-w_{3,1} && x_{8,2}-w_{1,2} &
      \\*\cline{3-9}
      & 
      && y_{4,1}-z_{3,1} && y_{2,1}-z_{4,1} && y_{7,2}-z_{6,2} &
      \\
      &
      && y_{5,1}-w_{3,1} && y_{5,1}-w_{4,1} && y_{8,2}-w_{6,2} &
      \\
      &
      && {\b z_{5,1}-w_{4,1}} && {\b z_{5,1}-w_{2,1}} && {\b z_{8,2}-w_{7,2}} &
      \\*\hline
      & 
      && x_{9,1}-y_{7,1}+z_{6,1}  && x_{7,1}-y_{6,1}+z_{9,1}  && x_{12,2}-y_{4,2}+z_{3,2}   &
      \\
      & \multirow{4}{*}{Round $3$}
      && x_{10,1}-y_{8,1}+w_{6,1} && x_{11,1}-y_{10,1}+w_{9,1}&& x_{13,2}-y_{5,2}+w_{3,2}   &
      \\
      &
      && x_{11,1}-z_{8,1}+w_{7,1} && -x_{8,1}-z_{10,1}+w_{6,1}&& x_{14,2}-z_{5,2}+w_{4,2}   &
      \\*\cline{3-9}
      & 
      && y_{11,1}-z_{10,1}+w_{9,1}&& -y_{8,1}-z_{11,1}+w_{7,1}&& y_{14,2}-z_{13,2}+w_{12,2} &
      \\*\hline
      & \textnormal{Round $4$}
      && x_{15,1}-y_{14,1}+z_{13,1}-w_{12,1} && x_{14,1}-y_{13,1}+z_{15,1}+w_{12,1} && x_{16,2}-y_{11,2}+z_{10,2}-w_{9,2} &
      \\*\IEEEeqnarrayrulerow
  \end{IEEEeqnarraybox}% }
\end{table}



